Stop Relying on No-Choice and Do not Repeat the Moves: Optimal, Efficient and Practical Algorithms for Assortment Optimization

We address the problem of active online assortment optimization problem with preference feedback, which is a framework for modeling user choices and subsetwise utility maximization. The framework is useful in various real-world applications including ad placement, online retail, recommender systems, fine-tuning language models, amongst many. The problem, although has been studied in the past, lacks an intuitive and practical solution approach with simultaneously efficient algorithm and optimal regret guarantee. E.g., popularly used assortment selection algorithms often require the presence of a `strong reference' which is always included in the choice sets, further they are also designed to offer the same assortments repeatedly until the reference item gets selected -- all such requirements are quite unrealistic for practical applications. In this paper, we designed efficient algorithms for the problem of regret minimization in assortment selection with \emph{Plackett Luce} (PL) based user choices. We designed a novel concentration guarantee for estimating the score parameters of the PL model using `\emph{Pairwise Rank-Breaking}', which builds the foundation of our proposed algorithms. Moreover, our methods are practical, provably optimal, and devoid of the aforementioned limitations of the existing methods. Empirical evaluations corroborate our findings and outperform the existing baselines.

==> alg_fr.tex <==
\section{Towards (Multiplicative) Faster Rates: Analzying \aa\ with \tf-$k$ Feedback}
\label{sec:alg_fr}

In this section, we consider the more general \tf-$k$\ feedback model (as defined in \cref{sec:prob}), where the learner gets to see a partial $k$-ranking of the items choices upon querying any set $S_t \subseteq [K]$, $k \in [m]$. 
%
The crux of our analysis lies in showing how one could exploit a $k$-length ranking towards obtaining a $k$-factor multiplicative improvement in the regret rate.
%
For brevity, we simply analyze the more general \utilm\ objective, but any careful reader would easily notice how our proposed techniques can be applied to \topm\ objective as well to get a similar $k$-factor multiplicative improvement in the regret rate. 
%

\subsection{Analyzing \utilm\ with \tf-$k$ feedback: Improved Regret with \emph{Rank-Breaking}}
\label{sec:alg_fr_util}

We will now see how a simple generalization of \algwf\, can lead us to a multiplicative improvement in the regret guarantee, leading to faster convergence with the general \tf-$k$ feedback. The idea is to use a simple yet powerful idea of \emph{Rank-Breaking} (\rb) to extract $k \choose 2$ pairwise comparisons from a single \tf-$k$ feedback. We provide a detailed discussion of \rb\ in \cref{sec:rb}. Just to summarize the idea intuitively, \rb\ is a way to extract pairwise comparisons from any ranking data, by considering each valid pairwise comparison out of the ranking information \citep{KhetanOh16,SueIcml+17}. 

Coming back to our problem setup, exploiting \rb, now we can essentially derive $k \choose 2$ valid pairwise comparisons of the items in $S_t$ per round $t$. This further leads to more accurate pairwise estimates $\hp_{ij}$ for each pair $(i,j)$, finally yielding a $k$-factor improved rate with careful analysis. Our complete algorithm is provided in \cref{alg:tf}. %in \cref{app:alg_wf_util} 
Further \cref{thm:utilm_tf} shows that it is provably optimal by proving an $O(\sqrt{KT}/k)$ regret performance for \tf-$k$ feedback.

%textbf{Main Idea to work with \tf-$k$ feedback...} \red{cleaning up required}

\noindent
\textbf{Rank-Breaking \citep{KhetanOh16}.}
Given any set $S$ of size $k$, if $\bsigma \in \bSigma_{S_m},\, (S_m \subseteq S,\, |S_m|=m)$ denotes a possible top-$m$ ranking of $S$, the \textit{Rank Breaking} subroutine considers each item in $S$ to be beaten by its preceding items in $\bsigma$ in a pairwise sense. 
% For instance, given a full ranking of a set of $4$ elements $S = \{a,b,c,d\}$, say $b \succ a \succ c \succ d$, Rank-Breaking generates the set of $6$ pairwise comparisons: $\{(b\succ a), (b\succ c), (b\succ d), (a\succ c), (a\succ d), (c\succ d)\}$. Similarly, given the ranking of only $2$ most preferred items say $b \succ a$, it yields the $5$ pairwise comparisons $(b, a\succ c),(b,a\succ d)$ and $(b\succ a)$ etc. 
% 
 See Algorithm \ref{alg:updt_win} for a detailed description of the Rank-Breaking procedure.


\noindent
\textbf{\algtf\ (\cref{alg:tf}): Generalizing \algwf\, for \tf-$k$ Feedback ($k \in [m]$).}
The main trick we use in modifying \algwf\, for \tf\ feedback is \textit{Rank Breaking}, which essentially extracts pairwise comparisons from subset-wise feedback as described below: %\red{complete + refine}.

Using \algupdt\, (Algorithm \ref{alg:updt_win}), our modified \algtf\, algorithm now essentially maintains the empirical pivotal preferences $\hp_{i0}$ for each item $i \in [K]$ by applying \textit{Rank Breaking} on the \tf\ feedback $\bsigma$ of each subsetwise play. 


%\vspace*{-28pt}
\begin{center}
\begin{algorithm}[h]
   \caption{\textbf{\algtf: \aa\ for PL model with \tf-$k$ Feedback}}
   \label{alg:tf}
\begin{algorithmic}[1]
   \STATE {\bfseries init:} $\tK \leftarrow K+1$, $[\tK]= [K] \cup\{0\}$, $\W \leftarrow [0]_{\tK \times \tK}$ %~~\red{($\alpha$ to be tuned)} %//Best candidate
   \FOR{$t = 1,2,3, \ldots, T$} %//Build $S_t$
	\STATE Set $\bN = \W + \W^\top$, and $\hat{\P} = \frac{\W}{\bN}$. Denote $N = [n_{ij}]_{\tK \times \tK}$ and $\hat P = [\hp_{ij}]_{\tK \times \tK}$.
	\STATE Define $u_{ij} = \hp_{ij} + \sqrt{\frac{2\ln t}{n_{ij}}}, \, \forall i,j \in [\tK], i\neq j$, $u_{ii} = \frac{1}{2}, \, \forall i \in [K]$. $\textbf{U} = [u_{ij}]_{K \times K}$ %(Set $\frac{x}{0} = 1$, $\forall x \in R$)
        \STATE $\htheta_i:= \nicefrac{\hp_{i0}}{1-\hp_{i0}}$, $\utheta_i:= \htheta_i + 4\sqrt{\frac{2\ln t}{n_{ij}}}$
        \STATE $S_{t} \leftarrow 
			\begin{cases}
				\text{Top-$m$ items from argsort}(\{\utheta_1,\dots,\utheta_K\}),\\
    ~~~~~~~~~~~~~~~~~~~~~~~\text{ for } \topm\ \text{ objective }\\
				\argmax_{S \subseteq [K] \mid |S| = m}\frac{\sum_{i \in S}\utheta_i}{\sum_{i \in S}\utheta_i +1},\\
    ~~~~~~~~~~~~~~~~~\text{ for } \utilm\ \text{ objective } 
			\end{cases}$
	\STATE Play $S_t$
        \STATE Receive the \tf-k\ $\sigma_t \in \Sigma_{S_t \cup \{0\}}$ (drawn as per \eqref{eq:prob_rnk1}) 
   \STATE Update: 
   \FOR {$k' = 1,2, \ldots, k)$}
   {\STATE \label{line:mm_rbk} $W(\sigma_t(k'),i) \leftarrow W(\sigma_t(k'),i) + 1 ~~ \forall i \in S_t\cup\{0\} \sm \sigma_t(1:k')$} %for all $k' = 1,2, \ldots, \min(|S_t|-1,m)$
   \ENDFOR   
   \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{center}
%\vspace*{-15pt}

\begin{lemma}[\red{Minimum Pairwise Comparisons with \tf-k\, feedback}]
\label{lem:ni0t_2}
For any item $i \in [K]$, and time $t \in [T]$
\[
Pr\biggn{ n_{i0,t} \leq \frac{n k (\theta_i + \theta_0)}{2(\theta_0 + \Theta_{S^*})}  \mid n_{i,t} = n } \leq \exp\bigg(- \frac{nk(\theta_i + \theta_0)}{8(\theta_0 + \Theta_{S^*})}\bigg).
\]

Further given any $\delta \in (0,1)$, for any $n \geq \frac{8(\theta_0 + \Theta_{S^*})}{k(\theta_0 + \theta_{i})}\ln \frac{1}{\delta}$, 
$Pr\biggn{ n_{i0,t} \leq \frac{n k (\theta_i + \theta_0)}{2(\theta_0 + \Theta_{S^*})}  \mid n_{i,t} = n } \leq \delta$.
\end{lemma}

\begin{proof}
%
The proof follows almost the same analysis of \cref{lem:ni0t}. The difference lies in the observation that: For any $i \in [K]$, 

\[
\E[n_{i0,T}] = \E[\sum_{t =1}^T \sum_{\ell = 1}^k \1(\sigma_t(\ell) \in \{i,0\})] \geq k\E\biggsn{\sum_{t = 1}^T \frac{(\theta_i+1)}{\Theta_{S_t}+1}\1(i \in S_t)}
\]

\begin{align*}
\E[n_{i0,t} \mid n_{i}(t) = n] &= \E[\sum_{\tau = 1}^t \sum_{\ell = 1}^k \1(i \in S_\tau) \1(\sigma_\tau(\ell) \in \{i,0\})) \mid n_{i}(t) = n]
\\  
& \geq \E[\sum_{\tau = 1}^t \sum_{\ell = 1}^k \1(i \in S_\tau) \frac{\theta_i + \theta_0}{\theta_0 + \Theta_{S_t}}) \mid n_{i}(t) = n]
\\
& \geq k\E[\sum_{\tau = 1}^t \1(i \in S_\tau) \frac{\theta_i + \theta_0}{\theta_0 + \Theta_{S^*}}) \mid n_{i}(t) = n ]
\\
& =  k\E[n_i(t) \mid n_{i}(t) = n]\frac{\theta_i + \theta_0}{\theta_0 + \Theta_{S^*}} = \frac{n k(\theta_i + \theta_0)}{\theta_0 + \Theta_{S^*}}.
\end{align*}

Now applying multiplicative Chernoff-Hoeffdings bound on $n_{i0,t}$ we get for any $\eta \in (0,1)$, 

\begin{align*}
Pr\Big( n_{i0,t} \le (1-\eta)\E[n_{i0,t}] \mid n_{i0,t} = n \Big) & \le \exp\bigg(- \frac{\E[n_{i0,t}]\eta^2}{2}\bigg) \le \exp\bigg(- \frac{n k(\theta_i + \theta_0)\eta^2}{2(\theta_0 + \Theta_{S^*})}\bigg), 
\end{align*}
this proves the first part of the claim for $\eta = 1/2$.
%
Further is easy to see that for the choice of $\eta = 1/2$, $\exp\bigg(- \frac{nk(\theta_i + \theta_0)\eta^2}{2(\theta_0 + \Theta_{S^*})}\bigg) \leq \delta$ for $n \geq \frac{8(\theta_0 + \Theta_{S^*})}{k(\theta_0 + \theta_{i})}\ln \frac{1}{\delta}$, proving the claim.
\end{proof}

\begin{restatable}[\algtf: Regret Analysis for \utilm\ with \tf-$k$\ Feedback]{theorem}{utilmtf}
\label{thm:utilm_tf}
Consider any instance of PL model on $K$ items with parameters $(\theta_1,\ldots,\theta_K)$ and let $w_i > 0$ be the weight associated to item-$i$, forall $i \in [K]$. Then given any finite time horizon $T$, the weighted regret of our proposed algorithm \algtf\ with \tf-$k$ ranking feedback is bounded by $\regu_T = O(\sqrt{\frac{KT}{k}\log KT})$. 
\end{restatable}

\begin{proof}[(Proof Sketch of \cref{thm:utilm_tf})]
Again recall
\begin{align*}
& Pr(|\hp_{t}(i,0)-p_t(i,0)| > \epsilon) \leq \exp(-n\epsilon^2) \\
& \implies \\
& Pr(|\hat \theta_i-\theta_i| > 4\epsilon) \leq Pr(|\hp_{t}(i,0)-p_t(i,0)| > \epsilon) 
\\
 & \hspace{1in} \leq \exp(-n\epsilon^2)
\end{align*}


Recall the definition of $\cW_S$ and $\cW_{S}^{\ucb}$ from the proof of \cref{thm:utilm_wf} for any subset $S \subseteq [K]$, and further recall from the weighted-UCB lemma \cref{lem:wtd_util}, we have: $\cW_{S}^{\ucb} \geq \cW_S, ~\forall S$.

Thus we have: $\cW_{S^*} \leq \cW_{S^*}^{\ucb} \leq \cW_{S_t}^{\ucb}$. 

\textbf{Case-1: Regret Bound for the \topm\ objective with \tf\ feedback:} The proof starts with the same intuition same we used for the \wf\ feedback, as:

\begin{align*}
   \regt_T & = \frac{1}{m} \sum_{t=1}^T \E[\Theta_{S^*} - \Theta(S_t)]  
    \leq \frac{1}{m} \sum_{t = 1}^T \E[\Theta_{S_t}^{\ucb} - \Theta_{S_t}]\\
    & \leq \frac{1}{m}\sum_{t=1}^T \E[\sum_{i\in S_t} \bign{\theta_i^{\ucb} - \theta_i}]\\
    & = \frac{1}{m}\sum_{i=1}^K \sum_{t = 1}^T \E[\bign{\theta_i^{\ucb} - \theta_i}\1(i \in S_t)]\\
    & \overset{(a)}{\leq} \frac{1}{m}\sum_{i=1}^K \E\biggsn{\sum_{t =1}^{n_i(T)} \frac{\sqrt{\log KT}}{\sqrt{n_{i0}(T)}} }\\
    &\overset{(\star)}{\leq} \frac{1}{m}\sum_{i=1}^K \E\biggsn{\sum_{t =1}^{ n_{i}(T)} \frac{\sqrt{\log KT}}{\sqrt{k n_{i}(T)/m}} }\\
    &\overset{(b)}\leq \frac{1}{m}\E\biggsn{\sum_{i=1}^K {\sqrt{\frac{m n_i(T)}{k} }\log KT} }\\
    & \overset{(c)}\leq \frac{1}{m}\E\biggsn{{m\sqrt{\frac{K T}{k}} \log KT} } = \sqrt{\frac{KT}{k}}\log (KT),
\end{align*}

where really the crucial step lies in $(\star)$ which shows in the case of \tf\ feedback, $\E[n_{i0}(T)] \geq \frac{k}{m}\E[n_i(T)]$ w.h.p. $(1-1/{KT})$ --- this is the crucial observation to gain the additional multiplicative improvement by the $\sqrt{k}$ ($k \in [m]$) factor. The rest of the inequalities $(a), (b), (c)$ follows the same logic as shown the proof of \cref{thm:topm_wf} for \wf\ feedback.

%where (a) follows by noting that $\E[n_{i0}(T)] \geq \frac{1}{m}\E[n_i(T)]$ w.h.p. $(1-1/{KT})$ at each round $t$ -- this is since the number of times either $i$ or $0$ won has to be at least $m$-factor of the total number of times item-$i$ was pulled. (b) and (c) simply follows by applying Cauchy's Schwarz Inequality with the additional observation that $\E[\sum_{i = 1}^K n_i(T)] \leq mT$.

\textbf{Case-2: Regret Bound for the \utilm\ objective:} Here again we need to carefully analyze the relation between $n_{i0}(T)$ and $n_i(T)$ to gain the $\sqrt{k}$-factor improvement in the regret bound. We again start by recalling that, $\cW_{S^*} \leq \cW_{S^*}^{\ucb} \leq \cW_{S_t}^{\ucb}$. Thus we can write:

\begin{align*}
   \regu_T & = \sum_{t=1}^T \E\bigsn{\cW_{S^*} - \cW(S_t)}  
    \leq \sum_{t = 1}^T \E\bigsn{\cW_{S_t}^{\ucb} - \cW_{S_t}}\\
    & \leq \sum_{t=1}^T \sum_{i\in S_t} \E\biggsn{\frac{\theta_i^{\ucb} - \theta_i}{(\Theta_{S_t}+1)}}\\
    & \leq \sum_{t=1}^T \sum_{i\in S_t} \E\biggsn{\frac{\sqrt{\log (KT)}}{(\Theta_{S_t}+1) \sqrt{n_{i0}(T)}}}\\
    & \leq \sum_{i=1}^K \E\biggsn{\sum_{t =1}^T \frac{\sqrt{\log (KT)}}{(\Theta_{S_t}+1)\sqrt{n_{i0}(T)}}\1(i \in S_t)}\\
    & = \sum_{i=1}^K \E\biggsn{\sum_{t =1}^T \frac{(\theta_i+1)\log (KT)}{(\Theta_{S_t}+1)\sqrt{n_{i0}(T)}}\frac{\1(i \in S_t)}{(\theta_i+1)}}\\
    & = \sum_{i=1}^K \E\biggsn{\sqrt{\frac{\log(KT)}{n_{i0}(T)}}\sum_{t =1}^{T} \frac{(\theta_i+1)}{\Theta_{S_t}+1}\1(i \in S_t)}\\
    & \overset{(a)}{\leq} \sum_{i=1}^K \E\biggsn{\sqrt{\frac{\log(KT)}{n_{i0}(T)}} \frac{n_{i0}(T)}{k}}\\
    & \overset{(b)}{\leq} \sqrt{\frac{2K T}{k} \log(KT)},
\end{align*}

where the important observation lies in noting that in this case (a) follows since for any $i \in [K]$, $\E[n_{i0}(T)] = \E[\sum_{t =1}^T \sum_{\ell = 1}^k \1(\sigma_t(\ell) \in \{i,0\})] \geq k\E\biggsn{\sum_{t = 1}^T \frac{(\theta_i+1)}{\Theta_{S_t}+1}\1(i \in S_t)}$. Further, another crucial observation is that (b) follows using Cauchy-Schwarz with the observation that $\sum_{i = 1}^K n_{i0}(T) \leq k2T$ for the \tf\ feedback.
This concludes the proof. 
%\red{Note this analysis works even if $w_i$s are positive in $[0,1]$ as we know for any valid $w_i \in [0,1]$s,} 
\end{proof}

\begin{rem}
Of course in general, \emph{Rank Breaking} may lead to arbitrarily inconsistent estimates of the underlying model parameters \citep{Az+12}. However, owing to the {\it IIA property} of the Plackett-Luce model, we get clean concentration guarantees on $p_{ij}$ using Lem. \ref{lem:pl_simulator}. This is precisely the idea used for obtaining the $\frac{1}{\sqrt k}$ factor improvement in the sample complexity guarantees of \algtf\, as analyzed in Theorem \ref{thm:utilm_tf}.
\end{rem}

\begin{rem}[Analyzing \topm\ Objective with \tf\ Feedback]
It is easy to see the above \rb\ idea easily applies to the \topm\ objective well and a similar proof analysis of \cref{thm:topm_wf} would lead to an $O(\sqrt{KT}/k)$ regret bound for the \topm\ objective with \tf\ feedback. We leave the details for the readers to work out this simpler setup. 
\end{rem}



==> expts.tex <==
\section{Experiments}
\label{sec:expts}
We run extensive simulations to compare our methods with the state-of-the-art MNL-Bandit algorithm \cite{assort-mnl} and provide a comparative empirical evaluation based on different experimental setups and choice of PL parameters $\btheta$. The details of our empirical results are given below: %of our proposed methods against the existing baselines.

\textbf{Algorithms.} 
\iffalse%%%%
We consider the general case where the no-choice item (Item $0$ with PL parameter $\theta_0$) is not necessarily the maximum, i.e., $\theta_0 \neq \max_{i \in [K]} \theta_i$. Thus, as motivated in \cref{alg:abi}, our proposed algorithm \algwf\ performs suboptimally in this general case, and hence we proposed the adaptive version \aalgwf. \textbf{(1).} For experimental analysis we use \aalgwf\, with an efficient \emph{adaptive-pivot}, where we use the estimated borda-winner (at time $t$) as the pivot, as follows:  
\begin{align*}
    & j_t \leftarrow \arg\max_{j \in [K]\cup{0}} \sum_{j \in [K]\cup\{0\}} \hp_{ij}\\
    & \htheta_{i,t}:= \nicefrac{\hp_{ij_t,t}}{1-\hp_{ij_t,t}}, \utheta_{i,t}:= \htheta_{i,t} + 4\sqrt{\frac{2\ln t}{n_{ij,t}}}\\
    & S_{t} \leftarrow 
			\begin{cases}
				\text{Top-$m$ items from argsort}(\{\utheta_{1,t},\dots,\utheta_{K,t}\}),\\
    ~~~~~~~~~~~~~~~~~~~~~~~\text{ for } \topm\ \text{ objective }\\
				\argmax_{S \subseteq [K] \mid |S| = m}\frac{\sum_{i \in S}w_i\utheta_{i,t}}{\sum_{i \in S}w_i\utheta_{i,t} +\theta_0},\\
    ~~~~~~~~~~~~~~~~~\text{ for } \utilm\ \text{ objective } 
\end{cases}
\end{align*}
\fi%%%%%%%%
We evaluated the relative performance of our main algorithm \textbf{(1). \aalgwf} (\cref{sec:abi}) with adaptive pivot, referred as \textbf{``Our Alg-1 (Adaptive Pivot)"}, with the following two algorithms:
%\textbf{\algwf\, with a general pivot:} This is a generalized version of our algorithm where we use the borda winner as a pivot item to estimate the PL parameters $\theta_i$.  
\textbf{(2). \algwf\,} (\cref{sec:alg_wi}) referred as \textbf{``Our Alg-2 (No-Choice Pivot)"},  
\textbf{(3). MNL-UCB:} The proposed algorithm in \cite{assort-mnl} in Algorithm-$1$.

\textbf{Different PL $(\btheta)$ Environments.}
We report our experiment results on two $\pl$ datasets with $K = 50$ items: (1) Arith$50$ with \pl\ parameters $\theta_i = 1 - (i-1)0.2, ~\forall i \in [50]$.
(2) Bad$50$ with \pl\ parameters $\theta_i = 0.6, ~\forall i \in [50]\sm\{25\}$ and $\theta_{25} = 0.8$. For simplicity of computing the assortment choices $S_t$, we assume $r_i = 1, ~\forall i \in [K]$.

\begin{rem}
Note in our PL environments, we set $\theta_{\max} = 1$ (to avoid scaling of $\regt$\, with ~$\theta_{\max}$). Since the choice probabilities of PL models are scale-independent, our choice of parameters is equivalent to assuming another choice model $(\theta'_1,\theta'_2,\ldots,\theta'_K)$, $\theta'_0 = 1$ and adjusting $\theta'_i = \nicefrac{\theta_i}{\theta_0}, ~\forall i \in [K]$. 
\end{rem}

In all the experiments, we report the averaged performance of the algorithms across $100$ runs.

\textbf{(1). Averaged Regret with weak NC $(\theta_{\max}/\theta_0 \gg 1)$ (Fig. \ref{fig:reg_wi}):} In our first set of experiments we report the average performance of the above three algorithms against \topm-\aa\, Regret ($\regt_T$) and \utilm-\aa\, Regret ($\regu_T$). We set $m=5$ and $\theta_0 = 0.01$ for this set of experiments. 
% and hence a regret guarantee of $O\big( \frac{n\ln T}{m} \big)$ as opposed to the $O\big( {n \ln T}\big)$ regret bound for both RUCB and BD. Fig. \ref{fig:reg} shows the results.
\vspace{-2pt}
\begin{figure}[h]
\vspace{-5pt}
\hspace{-10pt}
\includegraphics[trim={0cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/allin/arith50reg.png}
\hspace{-20pt}
\includegraphics[trim={3.2cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/allin/arith50util.png}
\hspace{-20pt}
\includegraphics[trim={3.2cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/allin/bad50reg.png}
\hspace{-10pt}
\includegraphics[trim={3.2cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/allin/bad50util.png}
\vspace{-20pt}
\caption{Averaged Regret for $m = 5$, $\theta_0 = 0.01$}
\label{fig:reg_wi}
\hspace{0pt}
\vspace{-15pt}
\end{figure}
%\vspace{-10pt}

\cref{fig:reg_wi} shows that our algorithm \aalgwf\, (with adaptive pivot) performs best, with a wide performance margin to the rest of the two algorithms, while our algorithm \algwf\, with no-choice (NC) pivot still outperforms MNL-UCB. But overall both of them perform poorly for $\theta_0 = 0.01$, as also expected since $\theta_{\max}$ is large compared to $\theta_0$ for these instances.

\textbf{(2). Averaged Regret vs No-Choice \pl\, Parameter $(\theta_0)$ (Fig. \ref{fig:reg_nc}):}
In this experiment, we evaluate the regret performance of our algorithm \aalgwf. We report the experiment on Artith$50$ \pl\ dataset and set the subsetsize $m = 6$, $\theta_0 = \{1, 0.5,0.1,0.05,0.01,0.005,0.001\}$. \cref{fig:reg_wi} shows, the performance gap between our algorithm \aalgwf\, (with adaptive pivot) increases with decreasing $\theta_0$ -- this is expected since the estimates of MNL-UCB strongly depends on the fact that $\theta_0$ needs to be maximum of $\{\theta_i\}_{i \in [K]}$ without which the algorithm performs increasingly suboptimaly due to poor estimation of the \pl\ parameters. 

\vspace{-2pt}
\begin{figure}[h]
\vspace{-5pt}
\hspace{-10pt}
\includegraphics[trim={0.4cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/vsnc/arith50reg1.png}
\includegraphics[trim={3.2cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/vsnc/arith50util.png}
\vspace{-20pt}
\caption{Comparative performances of the algorithms for varying strength of NC $(\theta_0)$ for $m = 5$}
\label{fig:reg_nc}
\hspace{0pt}
\vspace{-15pt}
\end{figure}
\vspace{-0pt}

%The additional experiments are moved to \cref{app:expts}.

%\iffalse%%%%%%%%%%%%%%%
\textbf{(3). Averaged Regret vs Length of the rank-ordered feedback ($k$) (Fig. \ref{fig:reg_tf}):}
We also run a thought experiment to understand the tradeoff between learning rate with $k$-length rank-ordered feedback, where given any assortment $S_t \subseteq [K]$ of size $m$, the learner gets to see the top-$k$ draws ($k\leq m$) from the PL model without replacement. Clearly, this is a stronger feedback than the winner (i.e. top-$1$ for $k=1$) feedback and one would expect a faster learning rate with increasing $k$ as the learner gets to observe more information from the PL model each time. We report the experiment on Artith$50$ \pl\ dataset and set the subsetsize $m = 30$ with $k = 1, 2, 4, 8$. As expected, we see a multiplicative reduction on both \topm-\aa\, Regret ($\regt_T$) and \utilm-\aa\, Regret ($\regu_T$) with increasing $k$, as reflected in \cref{fig:reg_tf}.

\vspace{-2pt}
\begin{figure}[h]
\vspace{-5pt}
\hspace{-10pt}
\includegraphics[trim={3.2cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/vsk/arith50reg.png}
\includegraphics[trim={3.2cm 0cm 0cm 0},clip,scale=0.1,width=0.245\textwidth]{./ICML24/img/vsk/arith50util.png}
\vspace{-20pt}
\caption{Tradofff: Averaged Regret vs length of the $k$ rank-ordered feedback for $k = 1,2,4,8$, $m = 30$}
\label{fig:reg_tf}
\hspace{0pt}
\vspace{-15pt}
\end{figure}
%\vspace{-10pt}
%\fi%%%%%%%%%%%%%%%%%


==> expts_long.tex <==
 \section{Detailed Experiments}
\label{app:expts}

%\red{Possibly to Appendix?}


\begin{center}
\begin{algorithm}[h]
   \caption{\textbf{\aa\ for PL model with DueLing UCB (\algwf-Modified)}}
   \label{alg:wf_mod}
\begin{algorithmic}[1]
   \STATE {\bfseries init:} $\tK \leftarrow K+1$, $[\tK]= [K] \cup\{0\}$, $\W \leftarrow [0]_{\tK \times \tK}$ %~~\red{($\alpha$ to be tuned)} %//Best candidate
   \FOR{$t = 1,2,3, \ldots, T$} %//Build $S_t$
	\STATE Set $\bN = \W + \W^\top$, and $\hat{\P} = \frac{\W}{\bN}$. Denote $N = [n_{ij}]_{\tK \times \tK}$ and $\hat P = [\hp_{ij}]_{\tK \times \tK}$.
        \STATE Define $u_{ij} = \hp_{ij} + \sqrt{\frac{2\ln t}{n_{ij}}}, \, \forall i,j \in [\tK], i\neq j$, $u_{ii} = \frac{1}{2}, \, \forall i \in [K]$. $\textbf{U} = [u_{ij}]_{K \times K}$ %(Set $\frac{x}{0} = 1$, $\forall x \in R$)
        \STATE $k = \argmax_i \Big\{\sum_{s=1}^{t-1} 1\{i = i_s^*\}\Big\}$.
        \STATE $\htheta_i:= \nicefrac{\hp_{ik}}{1-\hp_{ik}}$, $\utheta_i:= \htheta_i + 4\sqrt{\frac{2\ln t}{n_{ik}}}$
        \STATE $S_{t} \leftarrow 
			\begin{cases}
				\text{Top-$m$ items from argsort}(\{\utheta_1,\dots,\utheta_K\}),\\
    ~~~~~~~~~~~~~~~~~~~~~~~\text{ for } \topm\ \text{ objective }\\
				\argmax_{S \subseteq [K] \mid |S| = m}\frac{\sum_{i \in S}\utheta_i}{\sum_{i \in S}\utheta_i +1},\\
    ~~~~~~~~~~~~~~~~~\text{ for } \utilm\ \text{ objective } 
	\end{cases}$
	\STATE Play $S_t$
        \STATE Receive the \wf\ $i_t \in [\tK]$ (drawn as per \eqref{eq:prob_win}) 
   %\FOR {$k' = 1,2, \ldots, \min(|S_t|-1,m)$}
   {\STATE \label{line:mm_rb} Update:  $W(i_t,j) \leftarrow W(i_t,j) + 1 ~~ \forall j \in S_t\cup\{0\} \sm \{i_t\}$} for all $k' = 1,2, \ldots, \min(|S_t|-1,m)$
   %\ENDFOR   
   \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{center}


This section gives empirical performances of our algorithms (Alg. \ref{alg:mip} and  \ref{alg:rre}) and compare them with some existing preference learning algorithms. %We mostly restricted to pairwise feedback, unless otherwise specified, as most of the baselines only apply to dueling feedback ($q=2$). 
The details of the algorithms are given below: 

\textbf{Algorithms.} 
1%. \mip: Algorithm \algmip\, (Alg. \ref{alg:mip} as described in Sec. \ref{subsec:algmip}).
%2. \rre: Our proposed algorithm \algrre\, (Alg. \ref{alg:mip} as described in Sec. \ref{subsec:algrre}).
3  \ss: \emph{Self-Sparring} (independent beta priors on each arm) algorithm for multi-dueling bandits \citep{sui17} 
%4. \kss: Self-Sparring (thompson sampling based) algorithm for multi-dueling bandits \citep{sui17} 
%4.  \rucb: \emph{The Relative Upper Confidence Bound} algorithm for regret minimization in standard dueling bandits \cite{rucb}.
%5.  \pbo: \emph{Dueling-Thompson Sampling} algorithm for best arm identification problem in bayesian dueling bandits \cite{PBO}.
%
In every experiment, the performances of the algorithms are measured in terms of \emph{cumulative regret} (sec. \ref{eqn:reg}), averaged across $50$ runs, reported with standard deviation.%Before going to the details we first describe our experimental setup:

\textbf{Constructing Problem Instances.} 
%We first use preference functions with \emph{linear scores}: 
The difficulty of the instances depends on the difference of scores of the best and second best arms, which, in the hindsight, is actually governed by the `worst case slope' of the sigmoid function $\kappa$ (see the dependency of $\kappa$ in Thm. \ref{thm:reg_mip} or Thm. \ref{thm:reg_rre}), and also by the underlying problem parameter $\btheta^* \in \R^d$. 
%
So we used $3$ different \emph{linear score based} problem instances based on $3$ different characterizations of $\btheta^* \in \R^d$ (with $K$ arms and dimension $d$): 
\textbf{1. Easy $h(d,K)$}, 
\textbf{2. Extreme $e(d,K)$}, and
\textbf{3. Intermediate $m(d,K)$}, by suitably adjusting the norm $\|\btheta^*\|_2$. 
%The complete data generation procedure is given in Appendix \ref{app:expts}.
%For any instance, we first choose any arbitrary $\btheta^*$ in unit ball of dimension $d$ and subsequently scale its coordinates suitable to adjust the norm $\|\btheta^*\|$ in the desired range.
%
Also in all settings, the $d$-dimensional feature vectors (of the arm set) are generated as random linear combination of each arm to be a random linear combination of the d-dimensional basis vectors (for scaling issues of the item scores, we limit each instance vector to be within ball of radius $1$, i.e. $\ell_2$-norm upper bounded by $1$). %Following sections describe our different experimental results.

\textbf{Regret vs Time. } %We first analyse the regret the algorithms over time on $3$ different linear score environments: 
%For this experiment we fix $d = 10$ and $K = 50$. Fig. \ref{fig:reg_linn} shows both our algorithms \mip\, and \rre\, always outperform the rest, and their performance gets comparatively better with increasing hardness of the instances. As expected, \rucb \, performs the worst as by construction it fails to exploit the structure of underlying linear score based item preferences, due to the same reason \ss \, performs poorly as well (note we implement independent armed version of the \emph{Self-Sparring} algorithm \cite{sui17} for this case, and later the \emph{Kernelized} version for the case of non-linear item scores). On the contrary, \pbo\, performs reasonably well as it designed to exploit the underlying utility structures in the pairwise-preferences.


\iffalse 


\begin{figure}[H]
	\begin{center}
		\includegraphics[width=0.28\textwidth]{./plots/lin/h(10,50).png} \hspace{10pt}
		\includegraphics[width=0.28\textwidth]{./plots/lin/m(10,50).png}\hspace{10pt}
		\includegraphics[width=0.28\textwidth]{./plots/lin/e(10,50)_log.png}
		\vspace{-5pt}
		\caption{Average Cumulative Regret vs Time across algorithms on $3$ problem instances (linear score based preferences, $d=10, K=50$)}
		\label{fig:reg_linn}
	\end{center}
\end{figure}


%and also compare them with the {\it Self-Sparring} algorithm of \cite{Sui+17}, which is the only existing work applicable to our framework. %In all our experimental results, our proposed algorithm \textit{Battling-Duel} outperforms the rest, rightfully justifying the optimality of its regret guarantees as we discuss in Remark \ref{rem:bd_opt}. 
We first present the setup of our empirical evaluations:% are as follows:

\textbf{Algorithms.} We simulate the results on our two proposed algorithms (1). \algant \, and (2). \algestscr.
We also compare our ranking performance with the \emph{PLPAC-AMPR} method, the only existing method (to the best of our knowledge) that addresses the online PAC ranking problem, although only in the dueling bandit setup (i.e. $k = 2$).

\textbf{Ranking Performance Measure.} 
We use the popular pairwise \emph{Kendall's Tau ranking loss} \cite{Monjardet98} for measuring the accuracy of the estimated ranking $\bsigma$ with respect to the \br \, $\bsigma^*$ with an additive $\epsilon$-relaxation: %
%\vspace*{-22pt}
%\begin{align*}
%& d(\bsigma^*,\bsigma) = \frac{1}{{n \choose 2}}\sum_{i < j}\1\Big( (\sigma^*(i) - \sigma^*(j))(\sigma(i) - \sigma(j))  < 0 \Big)
%\end{align*}
$%\begin{align*}
d_{\epsilon}(\bsigma^*,\bsigma) = \frac{1}{{n \choose 2}}\sum_{i < j} (g_{ij} + g_{ji})$, where each $g_{ij} = \1\left( (\theta_i > \theta_j + \epsilon) \wedge(\sigma(i) > \sigma(j)) \right)$. %
%\Bigg[\1\Big( (\theta_i > \theta_j + \epsilon) \wedge(\sigma(i) > \sigma(j)) \Big)\\
% + \1\Big( (\theta_j > \theta_i + \epsilon) \wedge(\sigma(j) > \sigma(i)) \Big)\Bigg]
%$%\end{align*}
%%\vspace*{-22pt}
All reported performances are averaged across $50$ runs.

\textbf{Environments.}
We use four PL models: 1. {\it geo8} (with $n = 8$) 2. {\it arith10} (with $n = 10$) 3. {\it har20} (with $n = 20$) and 4. {\it arith50} (with $n = 50$). Their individual score parameters are as follows: \textbf{1. geo8:}
$
\theta_1=1$, and
$\frac{\theta_{i+1}}{\theta_{i}} = 0.875, ~\forall i \in [7]$. 
\textbf{2. arith10:} 
$\theta_1 = 1$ and $ \theta_{i} - \theta_{i+1} = 0.1, \, \forall i \in [9]$.
\textbf{3. har20:} $\theta = 1/(i), ~\forall i \in [20]$.
\textbf{4. arith50:} $\theta_1 = 1$ and $ \theta_{i} - \theta_{i+1} = 0.02, \, \forall i \in [9]$.

\iffalse%%%%%%%%%%%%%%%%%
%\subsection{Ranking Performance with Sample Complexity in the Dueling Setup ($k = 2$)}
%
%\vspace*{-20pt}
\begin{figure}[h!]
	\begin{center}
		\includegraphics[trim={0cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{geo8_all3.png}
		\hspace{0pt}
		%\vspace{10pt}
		\includegraphics[trim={0.cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{arith10_all3.png}
		\hspace{0pt}
		%\vspace{10pt}
		\includegraphics[trim={0cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{har20_all3.png}
		\hspace{0pt}
		%\vspace{10pt}
		\includegraphics[trim={0cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{arith50_all3.png}
		\vspace{-5pt}
		\caption{Ranking performance vs. sample size (\# rounds) with dueling plays ($k = 2$)}
		\label{fig:db}
		\vspace{-10pt}
	\end{center}
\end{figure}
\fi %%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Ranking with Pairwise Preferences ($k = 2$).} We first compare the above three algorithms with pairwise preference feedback, i.e. with $k = 2$ and $m = 1$ (WI feedback model). We set $\epsilon = 0.01$ and $\delta = 0.1$. Figure \ref{fig:db} clearly shows superiority of our two proposed algorithms over \emph{PLPAC-AMPR} \cite{Busa_pl} as they give much higher ranking accuracy given the sample size, rightfully justifying our improved theoretical guarantees as well (Theorem \ref{thm:batt_giant} and \ref{thm:est_thet}). Note that \emph{geo8} and \emph{arith50} are the easiest and hardest PL model instances, respectively; the latter has the largest $n$ with gaps $\theta_i - \theta_{i+1} = 0.02$. This also reflects in our experimental results as the ranking estimation loss being the highest for \emph{arith50} for all the algorithms, specifically  \emph{PLPAC-AMPR} very poorly till $10^4$ samples.

%\subsection{Performance with Sample Complexity in the Battling Setup (WI feedback)}

\iffalse%%%%%%%%%%%%%%%%%
\vspace*{-10pt}
\begin{figure}[H]
	\begin{center}
		\includegraphics[trim={0cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{har20_ant_k.png}
		\hspace{0pt}
		%\vspace{10pt}
		\includegraphics[trim={0.cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{arith50_ant_k.png}
		\vspace{-5pt}
		\caption{Ranking performance vs. subset size ($k$) with WI feedback ($m = 1$)} 
		\label{fig:varyk}
		\vspace{-10pt}
	\end{center}
\end{figure}
\fi%%%%%%%%%%%%%%%%%

\textbf{Ranking with Subsetwise-Preferences ($k>2$) with Winner feedback.} We next move to general subsetwise preference feedback $(k \ge 2)$ for WI feedback model (i.e. for $m = 1$) \footnote{\emph{PLPAC-AMPR} only works for $k = 2$ and is no longer applicable henceforth.}. We fix $\epsilon = 0.01$ and $\delta = 0.1$ and report the performance of \algant\,  on the datasets \emph{har20} and \emph{arith50}, varying $k$ over the range $4$ - $40$. As expected from Theorem \ref{thm:batt_giant} and explained in Remark \ref{rem:wi_null_k}, the ranking performance indeed does not seem to be varying with increasing subsetsize $k$ for WI feedback model for both PL models (Figure \ref{fig:varyk}).

%\subsection{Performance with Sample Complexity in the Battling Setup (TR feedback)}
%
%\vspace*{-10pt}
\iffalse%%%%%%%%%%%%%%%%%
\begin{figure}[H]
	\begin{center}
		\includegraphics[trim={0cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{har20_ant_m.png}
		\hspace{0pt}
		%\vspace{10pt}
		\includegraphics[trim={0.cm 0 0cm 0},clip,scale=0.25,width=0.23\textwidth]{arith50_ant_m.png}
		\vspace{-5pt}
		\caption{Ranking performance vs. feedback size ($m$) for fixed subset size ($k$)}
		\label{fig:varym}
		\vspace{-10pt}
	\end{center}
\end{figure}
\fi%%%%%%%%%%%%%%%%%
	%\vspace{-10pt}

\textbf{Ranking with Subsetwise-Preferences ($k>2$) with Top-rank feedback.} We finally report the performance of \algant\, (Algorithm \ref{alg:alg_ant_mod}) for top-$m$ ranking (TR) feedback model on two PL models: \emph{har20} (for $k = 20$) and \emph{arith50} (for $k = 45$), varying the range of $m$ from $2$ to $40$ (Figure \ref{fig:varym}). We set $\epsilon = 0.01$ and $\delta = 0.1$ as before. As expected, in this case indeed larger $m$ improves the ranking accuracy given a fixed sample size which reflects over theoretical guarantee of $\frac{1}{m}$-factor improvement of the sample complexity for TR feedback (Theorem \ref{thm:lb_pacpl_rnk} and Remark \ref{rem:1overm}).

%Clearly, {\it g10} is a harder model (to learn the Condorcet-winner), than {\it g1} as  the gap between the scores are very close to each other in $g10$ with the best and the second best item being only $0.2$ distance apart, whereas gap is $0.6$ for every suboptimal items in $g1$. The fact is reflected in our results too.


\fi%%%%%%%%%% ------------------------------------------

==> generalizations.tex <==
\section{Relaxations and Extensions}
\label{sec:extend}

\subsection{Generalizing \tf-$k$ to any $k$-length Partial Ranking}
\label{sec:nochoice}

- The same technique of rank breaking will give $k$-factor improvement!

\subsection{Relaxing `No-Choice' $(\theta_0)$}
\label{sec:nochoice}

- say the intuition and the final regret?

\subsection{Beyond PL: General RUM models}
\label{sec:beyondpl}

- say what is it and write the final theorem

The technical details are fairly straightforward to fill in given our proof analysis for the PL model (\cref{sec:alg_wi,sec:alg_fr}) and the pointers given above. Also we can do add all the proofs due to space constraints, but some additional details are provided in \cref{app:extend}. 


==> intreg.tex <==
\subsection{Generalizing Power of Internal Sleeping Regret}

In this section, we discuss, how $R_T^{\text{int}}$ generalizes the other existing notions of sleeping regret (\cref{sec:clsreg}).  

\paragraph{1. Internal Regret vs External Regret} We start by noting that following is a well-known result in the classical online learning setting~\citep{stoltz2005internal} (without sleeping).
 
 \begin{lemma}[Internal Regret Implies External Regret, \cite{stoltz2005internal}]
\label{lem:ext_int}
For any sequences $(\ell_t)$, $(S_t)$, and  any algorithm, 
$
    R_T^{\text{ext}}(k) = \sum_{i=1}^K R_T^{\text{int}}(i\to k)
$ for all $k \in [K]$.
\end{lemma}

The proof follows from the regret definitions. Thus any uniform upper-bound on the internal regret, implies the same bound for the external regret up to a factor $K$. The other direction is not true though!

\paragraph{2. Internal Sleeping Regret vs Ordering Regret}

\begin{lemma}[Internal Regret Implies Ordering  (for stochastic Losses)] 
\label{lem:implication}
Assume that the losses $(\ell_t)_{t\geq 1}$ are i.i.d..  Then, for any ordering $\sigma$, we have 
\[
    \E\big[R_T^{\text{ordering}}(\sigma)\big] \leq \sum_{i=1}^K \sum_{j \in D_i} \E\big[ R_T^{\text{int}}(i\to j) \big] \,. \vspace*{-5pt}
\]
where $D_i$ is the set of arms such that $\E[\ell_t(j)] \leq \E[\ell_t(i)]$. 
\end{lemma}
Therefore, any algorithm that satisfies $\E\big[ R_T^{\text{int}}(i\to j) \big]  \leq O(\sqrt{T})$, also satisfies $ \E\big[R_T^{\text{ordering}}(\sigma)\big] \leq O(\sqrt{T})$. 
The proof is deferred to the \cref{app:int_to_ord}.

\begin{remark}
\label{rem:adl_stcs}
An interesting research direction for the future would be to 
see if the sleeping internal regret also implies the ordering regret for adversarial losses and stochastic availabilities?  {Our experiments seem to point into this direction} (see \cref{app:expts}). Such a result would imply that any algorithm that can achieve sublinear regret w.r.t. sleeping internal regret $R_T^{\text{int}}$ (we in fact proposed such an algorithm in \cref{sec:alg_internal}, see SI-EXP3), would actually satisfy a best-of-both worlds guarantee. That is if either the losses or the availabilities are stochastic, the algorithm will incur a sublinear regret w.r.t. ordering regret $R_T^{\text{ordering}}$ as well. 
%
%If this is true, that would be a very interesting finding since then applying the same reduction to MAB idea, we can then have an $O(\sqrt T)$ regret algorithm for the adversarial preference and iid availability setting as well, which would give a Best-of-both world type algorithm for sleeping MAB or DB\footnote{That is a single algorithm that achieves $O(\sqrt{T})$ regret when either the losses/preferences or the availability sets are stochastic.}. \red{prune}
\end{remark}

\begin{remark}
On the other hand, it is well known that for adversarial losses, a small external regret does not imply a small internal regret~\cite{stoltz2005internal} even when $S_t = [K]$. But, when losses are stochastic and availabilities are adversarial, minimizing the ordering regret does control the internal regret (see \cref{app:int_to_ord}). 
\end{remark}
% \red{@Pierre: Can you add one more remark clarifying the other 2 directions we discussed yesterday: i.e. Ext regret does not imply Int regret when anything is adversarial and Ordering reg imply Intrnal only for iid loss and adv $S_t$? (we can add a proof also as discussed, may be in the appendix?)}



==> mab.tex <==
\section{SI-EXP3: AN ALGORITHM FOR INTERNAL SLEEPING REGRET} 
\label{sec:alg_internal}

We now propose an EXP3-based algorithm that guarantees sublinear sleeping internal regret. It is important to note that our algorithm works for the most challenging scenario of adversarial losses and availabilities, which includes stochastic settings (either losses or availabilities) as a special case. As proven in \cref{thm:internal}, our proposed algorithm SI-EXP3 achieves $\tilde O(\sqrt{KT})$ internal regret for any arbitrary sequence of losses $\{\ell_t\}_{t \in [T]}$ and availabilities $\{S_t\}_{t \in [T]}$. In addition, the generality of our internal regret (as shown in \cref{fig:rel}) implies $O(\sqrt{T})$ external regret in any scenario, as well as ordering regret for i.i.d losses, as explained in \cref{rem:reg_implication}.


%\paragraph{Related work} 
Our regret analysis is inspired from the construction of~\cite{stoltz2005incomplete} (see Section 3, Thm. 3.2) for the internal regret although the `sleeping component' or item non-avilabilities is not considered by \cite{stoltz2005incomplete}. 


Another relevant work is~\cite{blum2007external}, which designs an algorithm minimizing a variant of internal sleeping regret with a subtle difference: it considers time selection functions $I \in \mathcal{I} \subseteq \{0,1\}^T$ instead of sleeping actions. More precisely, the regret considered by \cite{blum2007external} is of the form\vspace*{-7pt}
$$
    \qquad \max_{I \in \mathcal{I}} \sum_{t=1}^T \big(\ell_t(k_t) - \ell_t(j)\big) \indic\{k_t = i, I(t)=1\}\,.
$$
Thus $R_T^{\text{int}}(i\to j)$ would correspond to the choice $I(t) = \indic\{j \in S_t\}$, but the dependence on the arm $j$ is not possible in their definition and makes the adaptation of their algorithm challenging. 
Moreover, their algorithm differs from ours and the one of \cite{stoltz2005incomplete} because it combines algorithms. In short, \cite{blum2007external} provides a reduction that needs $K$ instances of a no-external regret algorithm, that are combined by a meta-algorithm. 
% Very roughly, each $\mathcal{A}_i$ controls $\max_{j} R_T^{\text{int}}(i \to j)$, and the meta-algorithm controls $\max_{i} \max_{j} R_T^{\text{int}}(i\to j)$.
In contrast, we use a single instance of EXP3 to combine $K(K-1)$ fictitious experts. Each expert is in charge of controlling the internal regret $R_T^{int}(i\to j)$. No external regret algorithm is needed on the lower level. 
%
Because combining bandit algorithms is a difficult task (see e.g., \cite{agarwal2017corralling}), \cite{blum2007external} incurs suboptimal factors in $[K]$ (see their Thm. 11 which yields an internal regret of order $\smash{O(K \sqrt{TK \log K})}$), need extra assumptions (see their Lem. 10), and the adaptation of their analysis to sleeping is sophisticated. Note in particular that, their regret bound (Thm. 18) only holds in the full information setting, while their result on bandit feedback (Thm. 11) does not have the sleeping component.
%
We now describe our main algorithm, SI-EXP3, for optimizing Internal Sleeping Regret.

% \begin{remark}
% \red{@Pierre: Why Blum \& Mansour fails, and why it gives an additional K factor.}
% \end{remark}

\subsection{Algorithm: SI-EXP3} 
The Sleeping-Internal-EXP3 (SI-EXP3) procedure is a two-level algorithm. At round $t\geq 1$, the master algorithm forms a probability vector $p_t \in \Delta_K$ over the arms, which is used to sample the played action $k_t \sim p_t$. The vector $p_t$ is such that $p_t(i) = 0$ for any $i \notin S_t$. A subroutine, based on EXP3~\citep{Auer+02}, combines $K(K-1)$ sleeping experts indexed by $i \to j$, for $i \neq j$. Each expert aims to minimize the internal sleeping regret $R_T^{\text{int}}(i\to j)$. We detail below how to construct $p_t$. 

% \red{@P: If needed, you can move it to supp to save space}

\begin{algorithm}[h]
	\caption{SI-EXP3: Sleeping Internal Regret Algorithm for MAB}
	\label{alg:siexp}
	\begin{algorithmic}[1]	
		\STATE {\bfseries input:} Arm set: $[K]$, learning rate $\eta > 0$
            \STATE {\bfseries init:} $E := \{(i,j) \in [K]^2, i\neq j\}$\\
            \phantom{{\bfseries init: }}$\tilde q_1 \in \Delta_E$ uniform distribution on $E$
		\FOR{$t = 1, 2, \ldots, T$}
            \STATE Observe $S_t \subseteq [K]$ and define $q_t \in \Delta_E$ as in~\eqref{eq:defqt}
		% \FOR{$(i,j)$ in $E$} 
		% \STATE  
		% \ENDFOR
		\STATE Define $p_t \in \Delta_K$ by solving~\eqref{eq:defpt}
            \STATE Predict $k_t \sim p_t$ and observe $\ell_t(k_t)$
            \STATE Define $\hat \ell_t(k) = \frac{\ell_t(k)}{p_t(k)} \indic\{k = k_t\}$ for all $k \in [K]$
            \FOR{$(i,j) \in E$}
            \STATE Define $p_t^{i \to j} \in \Delta_K$ as in~\eqref{eq:defptijk}
            \STATE Define $\hat \ell_t(i\to j)$ as in~\eqref{eq:defhatellij}
		\STATE Update $\tilde q_{t+1}(i \to j) \propto \tilde q_t(i \to j) e^{- \eta \hat \ell_t(i\to j)}$
            \ENDFOR
		\ENDFOR  
		%\STATE Return $\bsigma'$
	\end{algorithmic} 
\end{algorithm} %\vspace{-10pt}

For any $i\neq j$, we denote by $p_t^{i\to j} \in \Delta_K$ the probability vector that moves the weight of  $p_t$ from $i$ to $j$, \vspace*{-5pt} 
\begin{equation}
    \label{eq:defptijk}
    p_t^{i\to j}(k) = \left\{
    \begin{array}{cc}
        0 & \text{if } k= i \\
        p_t(i) + p_t(j) & \text{if } k = j \\
        p_t(k) & \text{otherwise}
    \end{array} \right. \,.
\end{equation}
As usually considered in adversarial multi-armed bandits, for any active arm $i \in S_t$, we define the associated estimated loss $\hat \ell_t(i) := \ell_t(i)  \indic\{ i = k_t \}/p_t(i)$. 
Furthermore, by abuse of notation, we also define for any $i,j \in [K]$, $i\neq j$ the loss \vspace*{-5pt}
\begin{equation}
    \label{eq:defhatellij}
    \hat \ell_t\big( i \to j \big) := \left\{ 
    \begin{array}{ll}
        \sum_{k=1}^K p_t^{i \to j}(k) \hat \ell_t(k) & \text{if } j \in S_t \\
         \ell_t(k_t) & \text{otherwise}
    \end{array} \right.\!\!.
\end{equation}
The subroutine then computes the exponential weighted average of the experts $i \to j$, by forming the weights \vspace{-7pt}
\begin{equation}
    \hspace*{-10pt} \tilde q_t(i\to j) := \frac{\exp\Big( - \eta \sum_{s=1}^{t-1}  \hat \ell_s (i\to j) \Big)}{\sum_{i'\neq j '}\exp\Big( - \eta \sum_{s=1}^{t-1}  \hat \ell_s(i' \to j') \Big) } \,.
    \label{eq:deftildeqt}
\end{equation}
To avoid assigning mass from an active item $i$ to an inactive $j \notin S_t$, the subroutine then normalizes those weights so that sleeping experts get $0$ mass
\begin{equation}
    \label{eq:defqt}
     q_t(i \to j) := \frac{\tilde q_t(i \to j) \indic\{j \in S_t\} }{\sum_{i'\neq j'} \tilde q_t(i'\to j') \indic\{j' \in S_t\}} \,.
\end{equation}
Finally, the master algorithm forms $p_t \in \Delta_K$ by solving the linear system
\begin{equation}
    \label{eq:defpt}
    p_t = \sum_{i \neq j} p_t^{i \to j} q_t(i \to j) \,.
\end{equation}
The existence and the practical computation of such a $p_t$ is an application of Lemma 3.1 of~\cite{stoltz2005incomplete}. Similarly to \cite{blum2007external} and \cite{stoltz2005incomplete}, the space and per-round time complexities of SI-EXP3 are $O(K^2)$ and $O(K^3)$ respectively. 
The bottleneck is the above fixed point resolution of $p_t$ in \eqref{eq:defpt}. 


\subsection{Regret Analysis of SI-EXP3} 
We now analyze the sleeping internal regret guarantee of \cref{alg:siexp} (\cref{thm:internal}), and also the implications to other notions of sleeping regret (\cref{rem:reg_implication}).

\begin{theorem} 
\label{thm:internal}
Consider the problem of Sleeping MAB for arbitrary (adversarial) sequences of losses $\{\ell_t\}$ and availabilities $\{S_t\}$. Let $T \geq 1$ and $\smash{\eta^2 = (\log K)/ \big(2 \sum_{t=1}^T |S_t|\big)}$. Assume that $0\leq \ell_t(i)\leq 1$ for any $i \in S_t$ and $t \in [T]$. Then, \vspace*{-7pt}
\[
    \E\big[R_T^{\text{int}}(i\to j)\big] \leq 2  \sqrt{2 \log K \sum_{t=1}^T |S_t|} \leq 2 \sqrt{2 T K \log K} \,,
\]
for all $i \neq j$ in $[K]$.
\end{theorem}

The proof is postponed to \cref{app:proof_thm}. The learning rate $\eta$ can be calibrated online at the price of a constant factor by choosing a time-varying learning rate $\smash{\eta_t^2 = (\log K)/ \big(2 \sum_{s=1}^t |S_s|\big)}$ or by using the doubling-trick technique~\citep{cesa2006prediction}.

\begin{remark}
	\label{rem:reg_implication}
 The above theorem also implies a bound of order $O(K\sqrt{KT \log K})$ for the external sleeping regret by~\cref{lem:ext_int} and $O(K^2 \sqrt{KT \log K})$ for the ordering regret when the losses are i.i.d. by~\cref{lem:implication}. SI-EXP3 is the first to simultaneously achieve order-optimal \emph{sleeping external regret} for fully adversarial setup as well as \emph{ordering regret} for stochastic losses and this was possible owning to the versatility of \emph{Sleeping Internal Regret} as summarized in \cref{fig:rel}.
\end{remark}




==> old_alg_bi.tex <==
\section{Analzying \aa\ with \wf\, Feedback}
\label{sec:alg_wi}

In this section, we describe algorithms for \wf\, Feedback for our two objectives: \topm \ and \utilm. The algorithmic ideas are very similar for both objectives. The crux of our novelty lies in our parameter estimation technique which shows how one can maintain estimate pairwise scores of $p_{ij} = \frac{\theta_i}{\theta_i + \theta_j}$ for each item $i \in [K]$, against a fixed item (item-$0$ in this case). We identified a key lemma in \cite{SG19} to ``Deviations of pairwise win-probability estimates for PL model" (see Lemma 1, \cite{SG19}). We describe the algorithm details in the next section and analyze its regret guarantees for both \topm\ and \utilm \ objective, respectively in \cref{thm:topm_wf} and \cref{thm:utilm_wf}.

\subsection{Algorithm Design for \wf\ Feedback}
\label{subsec:alg_wi_detail}

\textbf{Main Idea. } 
A key idea behind our proposed algorithms is to estimate the relative strength of each item with respect to a fixed item, termed as the \emph{pivot-item}. We choose the pivot item to be the `no-choice item' (item-$0$ with score $\theta_0$) in this case since it is a default item in every set. Now using Lemma 1 of  \cite{SG19} we observe that this equips us to maintain a pairwise score of each item-$i$ against the pivot, precisely $p_{i0} = \frac{\theta_i}{\theta_i + \theta_0}, ~\forall i \in [K]$. For this we precisely in the following steps:

\textbf{Maintaining Pairwise Estimates. }
Maintains a pairwise preference matrix $\bhP \in [0,1]^{n \times n}$, whose $(i,j)$-th entry $\hp_{ij,t}$ records the empirical probability of $i$ having beaten $j$ in a pairwise duel, and a corresponding upper confidence bound $p^{\text{ucb}}_{ij}$ for each pair $(i,j)$.
%$p^{\text{ucb}}_{ij} = \hp_{ij} + \sqrt{\frac{\alpha\ln t}{N(i,j)}}$. 
%At any round $t$, it plays a subset $S_t \subseteq [n], \, |S_t| \in [k]$ using the \emph{Max-Min} set building rule \algbld\, (see Alg. \ref{alg:bld}), receives \tf\, $\sigma_t \in \Sigma_{S_t}^m$ from $S_t$, and updates the $\hp_{ij}$ entries of pairs in $S_t$ by applying \rb\, (Line $10$). 

\textbf{Estimate PL scores $\hat \theta$ from Pairwise Estimates. }
Our algorithm \algwf\, maintains pairwise score estimates $\hp_{i0,t}$ for each item $i \in [K]$ with respect to the pivot element $0$ (no-choice), and further by deriving intuition from \cref{lem:pl_simulator} we also assure fast concentration to $p_{ij}$ for each pair $(i,j) \in [\tK]\times[\tK]$, where we define $\tK = [K]\cup\{0\}$. We estimate $\hp_{ij,t}:= \frac{\w_{ij,t}}{n_{ij,t}}$, where $w_{ij,t}$ denotes the number of pairwise wins of item-$i$ over $j$ upon rank breaking, and $n_{ij,t} = w_{ij,t}+w_{ji,t}$ being the number of times $(i,j)$ has been compared after rank breaking. 
The algorithm further maintains UCB estimates, $p^{\text{ucb}}_{ij,t}$, of each $(i,j)$ pair, defined as $p^{\text{ucb}}_{ij,t}:= \hp_{ij,t} + c_{ij,t}$; where $c_{ij,t}:= \frac{\log T}{\sqrt{n_{ij,t}}}$ denotes the confidence of the pairwise estimate $p_{ij} = \frac{\theta_i}{\theta_i + \theta_j}$. 
Since our parameter estimation technique relies on maintaining pairwise duels $W(i,0)$ of each item $i \in [K]$ vs item-$0$, we name it as \algwf\. The complete algorithm is described in \cref{alg:wf}.

%\vspace*{-28pt}
\begin{center}
\begin{algorithm}[h]
   \caption{\textbf{\aa\ for PL model with DueLing UCB (\algwf)}}
   \label{alg:wf}
\begin{algorithmic}[1]
   \STATE {\bfseries init:} $\tK \leftarrow K+1$, $[\tK]= [K] \cup\{0\}$, $\W \leftarrow [0]_{\tK \times \tK}$ %~~\red{($\alpha$ to be tuned)} %//Best candidate
   \FOR{$t = 1,2,3, \ldots, T$} %//Build $S_t$
	\STATE Set $\bN = \W + \W^\top$, and $\hat{P} = \frac{\W}{\bN}$. Denote $N_t = [n_{ij}]_{\tK \times \tK}$ and $\hat P = [\hp_{ij}]_{\tK \times \tK}$.
        \STATE Define $p^{\text{ucb}}_{ij} = \hp_{ij} + \sqrt{\frac{2 { \hp_{ij}(1-\hp_{ij})} x}{n_{ij}}} + \frac{3x}{n_{ij}}, \, \forall i,j \in [\tK], i\neq j$, $p^{\text{ucb}}_{ii} = \frac{1}{2}, \, \forall i \in [K]$. $\textbf{U} = [p^{\text{ucb}}_{ij}]_{K \times K}$ %(Set $\frac{x}{0} = 1$, $\forall x \in R$)
        \STATE $\utheta_i:= p^{\ucb}_{i0}/(1-p^{\ucb}_{i0})_+ $
        \STATE $S_{t} \leftarrow 
			\begin{cases}
				\text{Top-$m$ items from argsort}(\{\utheta_1,\dots,\utheta_K\}),\\
    ~~~~~~~~~~~~~~~~~~~~~~~\text{ for } \topm\ \text{ objective }\\
				\argmax_{S \subseteq [K] \mid |S| = m}\frac{\sum_{i \in S}\theta_i^{\ucb}}{\sum_{i \in S}\theta_i^{\ucb} +1},\\
    ~~~~~~~~~~~~~~~~~\text{ for } \utilm\ \text{ objective } 
	\end{cases}$
	\STATE Play $S_t$
        \STATE Receive the \wf\ $i_t \in [\tK]$ (drawn as per \eqref{eq:prob_win}) 
   %\FOR {$k' = 1,2, \ldots, \min(|S_t|-1,m)$}
   {\STATE \label{line:mm_rb} Update:  $W(i_t,j) \leftarrow W(i_t,j) + 1 ~~ \forall j \in S_t\cup\{0\} \sm \{i_t\}$} for all $k' = 1,2, \ldots, \min(|S_t|-1,m)$
   %\ENDFOR   
   \ENDFOR
\end{algorithmic}
\end{algorithm}
\end{center}
%\vspace*{-15pt}


%\red{Todo (Oct 31st)}

%\red{1. Clean up the existing results. (2). Check how the above algorithm is performing empirically over MNL bandits (3) For theoretical analysis and see an improvement over MNL, ideally we want the above algorithm with doubling trick + we want to get rid of the assumption that NC has the highest $\theta_0$ (4) We should also think of deriving gap-dependent bounds. Plan this to be on ArXiv by Nov end.}

\begin{rem}
Say the rate is optimal since even MAB problem has this rate, which is a much simpler objective to compared to the std one which competes simply against a fixed `best' item, and even tha problem has the rate $\Omega(\sqrt{KT})$ \cite{Auer00,Auer+02}. 
\end{rem}

\subsection{Analysis: \topm\ Objective with \wf\ Feedback.}
\label{sec:alg_wi_analys}

We will start this section by defining some notations for the exposition:

\begin{align*}
    \hat p_{ij,t} & = \frac{w_{ij,t}}{n_{ij,t}}  \\
    p^{\text{ucb}}_{ij,t} & = \hat p_{ij,t} + \sqrt{\frac{2 \hat p_{ij,t}(1-\hat p_{ij,t}) x}{n_{ij,t}}} + \frac{3x}{n_{ij,t}} \\
    \theta_{i,t}^{\text{ucb}} & = \frac{p_{i0,t}^{\text{ucb}}}{(1 - p_{i0,t}^{\text{ucb}})_+} 
\end{align*}

\begin{lemma} 
\label{lem:pconc}
For any $T\geq 1$ and $x >0$ with probability at least $1-\beta(x,T)$ (see \citet[Thm. 1]{audibert2009exploration}),
\begin{equation}
    p_{ij} \leq p_{ij,t}^{\text{ucb}} \leq  p_{ij} + 2\sqrt{\frac{2 p_{ij}(1-p_{ij}) x}{n_{ij,t}}} + \frac{11x}{n_{ij,t}} \,, 
    \label{eq:ucb_p1}
\end{equation}
simultaneously for all $t \geq [T]$.
\end{lemma}

\begin{proof}
    Let $T\geq 1$, $x >0$ and $i,j\in [K]$. Then, noting that given $n_{ij,t}$, $w_{ij,t}$ is a binomial random variable with parameters $n_{ij,t}, p_{ij}$, we may apply Thm. 1 of \cite{Audibert+10} to get that, with probability at least $1-\beta(x,T)$, simultaneously for all $t \in [T]$, 
    \begin{equation}
        \big| \hat p_{ij,t} - p_{ij} \big| \leq \sqrt{\frac{2 \hat p_{ij,t}(1-\hat p_{ij,t})x}{n_{ij,t}}} + \frac{3x}{n_{ij,t}} \,.
        \label{eq:ucb_p}
    \end{equation}
    Note that the inequality holds true although $n_{ij,t}$ is a random variable. This, shows the first inequality
    \[
        p_{ij} \leq p_{ij,t}^{\text{ucb}} \,.
    \]
    For the second inequality, \eqref{eq:ucb_p} implies
    \begin{align}
        p_{ij,t}^{\text{ucb}} 
            & = \hat p_{ij,t} + \sqrt{\frac{2 \hat p_{ij,t}(1-\hat p_{ij,t}) x}{n_{ij,t}}} + \frac{3x}{n_{ij,t}} \nonumber \\
            & \leq  p_{ij} + 2\sqrt{\frac{2 \hat p_{ij,t}(1-\hat p_{ij,t})x}{n_{ij,t}}} + \frac{6x}{n_{ij,t}} \,.\label{eq:ucb_var}
    \end{align}
    Furthermore, because $x \mapsto x(1-x)$ is 1-Lipschitz on $[0,1]$, we have
    \begin{align*}
        \big|\hat p_{ij,t}(1-\hat p_{ij,t}) & - p_{ij}(1-p_{ij})\big| \leq  \big| \hat p_{ij,t} - p_{ij} \big| \\
            & \stackrel{\eqref{eq:ucb_p}}{\leq} \sqrt{\frac{2 \hat p_{ij,t}(1-\hat p_{ij,t})x}{n_{ij,t}}} + \frac{3x}{n_{ij,t}} \,.
    \end{align*}
    Therefore,
    \begin{align*}
        \hat p_{ij,t}(1-\hat p_{ij,t}) 
            & \leq p_{ij}(1-p_{ij}) + \sqrt{\frac{2 \hat p_{ij,t}(1-\hat p_{ij,t})x}{n_{ij,t}}} + \frac{3x}{n_{ij,t}} \\
            & \leq \bigg(\sqrt{p_{ij}(1-p_{ij})} + \sqrt{\frac{3x}{n_{ij,t}}}\bigg)^2 \,,
    \end{align*}
    which yields
    \begin{equation}
        \sqrt{\hat p_{ij,t}(1-\hat p_{ij,t}}) \leq \sqrt{p_{ij}(1-p_{ij})} + \sqrt{\frac{3x}{n_{ij,t}}}\,.\label{eq:ucb_std}
    \end{equation}
    Plugging back into~\eqref{eq:ucb_var}, we get
    \[
        p_{ij,t}^{\text{ucb}} \leq 2\sqrt{\frac{2  p_{ij}(1- p_{ij})x}{n_{ij,t}}} + \frac{11x}{n_{ij,t}}\,.
    \]
\end{proof}

\begin{lemma} 
\label{lem:tconc}
Let $t\in [T]$, $i \in [K]$. Then, if \eqref{eq:ucb_p1} holds, then $\theta_i \leq \theta_{i,t}^\text{ucb}$. Furthermere, if  $n_{i0,t} \geq 6\sqrt{2} x (1+\theta_i)$ we also have
\[
    \theta_i \leq \theta^{\text{ucb}}_{i,t} \leq \theta_i +  4(1+\theta_i)\sqrt{\frac{2 \theta_i x}{n_{i0,t}}} + \frac{22x(1+\theta_i)^2}{n_{i0,t}} \,.
\]
\end{lemma}

\begin{proof}
Let $t \in [T]$ and $i \in [K]$ and assume that~\eqref{eq:ucb_p1} holds true. Define the function $f:x\mapsto x/(1-x)_+$ on $[0,1]$ (with the convention $f(1) = +\infty$), so that $\theta_{i,t}^{\text{ucb}} = f(p_{i0,t}^{\text{ucb}})$ and $\theta_i = f(p_{i0})$. Because $f$ is non-decreasing, and $p_{i0,t}^{\text{ucb}} \geq p_{i0}$, we have
\[
    \theta_{i,t}^{\text{ucb}} \geq \theta_i \,.
\]
Furthermore, denote 
\begin{align*}
    \Delta_{i,t} & :=  2\sqrt{\frac{2 p_{ij}(1-p_{ij}) x}{n_{i0,t}}} + \frac{11x}{n_{i0,t}} \\
        & = 2\sqrt{\frac{2 \theta_i x}{(1+\theta_i)^2 n_{i0,t}}} + \frac{11x}{n_{i0,t}} \,.
\end{align*}
If $n_{i0,t} \geq 6\sqrt{2} x (1+\theta_i)$, we have
\begin{align*}
    (1+\theta_i)  \Delta_{i,t} & \leq 2 \sqrt{\frac{2\theta_i x}{n_{i0,t}}} + \frac{12x(1+\theta_i)}{n_{i0,t}}\\
    & \leq 2 \sqrt{\frac{2(1+\theta_i) x}{n_{i0,t}}} + \frac{12 x(1+\theta_i)}{n_{i0,t}}  \leq \frac{1}{2} \,,
\end{align*}
and similarly
\begin{align*}
    p_{i0,t} + \Delta_{i,t}  = \frac{\theta_i}{1 + \theta_i} + \Delta_{i,t} = \frac{\theta_i + 1/2}{\theta_i + 1} < 1. 
\end{align*}
Thus, because $f$ is non-decreasing
\begin{align*}
    \theta_{i,t}^{ucb} - \theta_i
        & = f(p_{i0,t}^{\text{ucb}}) - f(p_{i0})  \\
        & \stackrel{\eqref{eq:ucb_p}}{\leq} f\big(p_{i0,t} +  \Delta_{i,t}\big) - f(p_{i0}) \\
        & = \frac{p_{i0} +  \Delta_{i,t}}{1-p_{i0} -  \Delta_{i,t}} - \frac{p_{i0}}{1-p_{i0}} \\
        & = \frac{ \Delta_{i,t}}{(1-p_{i0})(1-p_{i0}- \Delta_{i,t})}\\
        & = \frac{(1+\theta_i)^2  \Delta_{i,t}}{1- (1+\theta_i) \Delta_{i,t}}\\
        & \leq  2 (1+\theta_i)^2  \Delta_{i,t} \,.
\end{align*}
and concludes the proof. 
\end{proof}

\begin{rem}[Choice of $x$ in \cref{lem:pconc}]
\label{rem:conc}
Note from \citet[Thm. 1]{audibert2009exploration}, we have 
\[
\beta(x,t) = 3 \underset{1 < \alpha \leq 3}{\text{inf}}\min \biggn{ \frac{\log t}{\log \alpha},t}e^{-x/\alpha}.
\]
Thus as $\alpha \to 1$, $\beta(x,t) \leq 3t e^{-x}$. Thus given any fixed $\delta > 0$, we can choose $x = \log \frac{3t}{\delta}$ to ensure $\beta(x,t) \leq \delta$. 
\end{rem}

Using \cref{rem:conc} and combining the results from \cref{lem:pconc} and \cref{lem:tconc}, we get that:

\begin{corollary} 
\label{lem:tconc}
Consider any fixed $t\in [T]$, $i \in [K]$ and $\delta > 0$. Furthermore, if $n_{i0,t} \geq 6\sqrt{2}(1+\theta_i) \log \bign{3t/\delta}$. Then with probability at least $1-\delta$
\[
    \theta_i \leq \theta^{\text{ucb}}_{i,t} \leq \theta_i +  4(1+\theta_i)\sqrt{\frac{2 \theta_i \log \frac{3t}{\delta}}{n_{i0,t}}} + \frac{22(1+\theta_i)^2 \log \frac{3t}{\delta}}{n_{i0,t}} \,.
\]
\end{corollary}

\begin{restatable}[\algwf: Regret Analysis for \topm\ with \wf\ Feedback]{theorem}{topmwf}
\label{thm:topm_wf}
Consider any instance of PL model on $K$ items with parameters $(\theta_1,\ldots,\theta_K)$. Then given any finite time horizon $T$, the regret of our proposed algorithm \algwf\ is bounded as $\regt_T = O(\sqrt{KT}\log KT)$. 
\end{restatable}

\begin{proof}[Proof Sketch of \cref{thm:topm_wf}]
Let us define for any $S \subseteq [K]$,
\[
\Theta_S = \sum_{i \in S}\theta_i, ~~\text{ and }~~ \Theta_S^{\ucb}:= \sum_{i \in S}\theta_i^{\ucb}.
\]

To bound the regret, note the expected number of times either $i$ or $0$ wins overall $T$ rounds are:
%
$\E[n_{i0,T}] = \sum_{t = 1}^T\frac{\theta_0+\theta_i}{\theta_{S_t}+1}$. %\red{--- will be crucial to remove the denominator term for us, since note our concentration will also happen in terms of $[n_{i0,T}]$}
%
Further we have: $\Theta_{S^*} \leq \Theta_{S^*,t}^{\ucb} \leq \Theta_{S_t,t}^{\ucb}$, where the second inequality follows from our subset selection rule of \cref{alg:wf}. 
%
Now let us define a good event: 
%
$\cG:= \{ \forall i \in [K], \text{ if } n_{i0,t} \geq 6\sqrt{2}(1+\theta_i) \log \bign{3t/\delta}
\text{ then }
\theta^{\text{ucb}}_{i,t} -\theta_i \leq \theta_i +  4(1+\theta_i)\sqrt{\frac{2 \theta_i \log \frac{3t}{\delta}}{n_{i0,t}}} + \frac{22x(1+\theta_i)^2}{n_{i0,t}}, \forall t \in [T] \}$, i.e. $\cG$ implies the concentration of \cref{lem:tconc} holds for all $i \in [K]$.

Clearly, taking union bound over all $i \in [K]$, 
$
P\bign{\cG} \leq \delta K$. Let us choose $\delta = 1/KT$.

Let us denote by $\bar n_{i0} = 6\sqrt{2}(1+\theta_i) \log \bign{3t/\delta}$. The claim now follows noting \red{change}: 

%\textbf{Case-1: Regret Bound for the \topm\ objective:} Applying the above lemma we get:



\begin{align*}
    \E&[\regt_T \mid \cG] = \frac{1}{m} \sum_{t=1}^T \E[\Theta_{S^*} - \Theta_{S_t} \mid \cG] = \frac{1}{m} \sum_{t=1}^T \E[\Theta_{S^*} - \sum_{i \in S_t}\theta_i \mid \cG] = \frac{1}{m} \sum_{t=1}^T \E\biggsn{\sum_{i \in S_t}(\Theta_{S^*}/m - \theta_i) \mid \cG}   \\
    & =  \frac{1}{m} \E\biggsn{\sum_{i=1}^K\sum_{t = 1}^T (\Theta_{S^*}/m - \theta_{i})\1(i \in S_t) \mid \cG}
    \\
    & = \frac{1}{m} \E\biggsn{\sum_{i=1}^K\sum_{n = 1}^{n_i(T)} (\Theta_{S^*}/m - \theta_{i}) \mid \cG}
    \\
    & = \frac{1}{m} \E\biggsn{\sum_{i=1}^K\sum_{n = 1}^{\bar n_{i0}} (\Theta_{S^*}/m - \theta_{i}) +
    \sum_{i=1}^K\sum_{n = \bar n_{i0} + 1}^{n_i(T)} (\Theta_{S^*}/m - \theta_{i}) \mid \cG}
    \\
    & \leq \frac{6\sqrt{2}\theta_{\max}\log \bign{3t/\delta} \sum_{i = 1}^K (1+\theta_{i})}{m} +
    \frac{1}{m} \E\biggsn{\sum_{t = 1}^{T}\sum_{i \in S_t} (\Theta_{S^*} - \theta_{i})\1(n_i(t) > \bar n_{i0}) \mid \cG}
    \\
    & \leq \frac{6\sqrt{2}\theta_{\max}\log \bign{3t/\delta} \sum_{i = 1}^K (1+\theta_{i})}{m} + \frac{1}{m} \sum_{t = 1}^T\biggsn{\sum_{i \in S_t} (\theta_{i,t}^{\ucb} - \theta_{i,t})\1(n_i(t) > \bar n_{i0}) \mid \cG } ~(\text{as } \Theta_{S^*} \leq \Theta_{S^*,t}^{\ucb} \leq \Theta_{S_t,t}^{\ucb}),\\
    & \leq C_0 + \frac{1}{m} \sum_{t = 1}^T\biggsn{\sum_{i \in S_t} (\theta_{i,t}^{\ucb} - \theta_{i,t})\1(n_i(t) > \bar n_{i0}) \mid \cG } ~ \biggn{\text{where } C_0 = \frac{6\sqrt{2}\theta_{\max}\log \bign{3t/\delta} \sum_{i = 1}^K (1+\theta_{i})}{m}}\\
    & \leq C_0 + \frac{1}{m}\sum_{t=1}^T \E[\sum_{i\in S_t} \bign{\theta_{i,t}^{\ucb} - \theta_i}\mid \cG] \\
    & = \frac{1}{m}\sum_{i=1}^K \sum_{t = 1}^T \E[\bign{\theta_{i,t}^{\ucb} - \theta_i}\1(i \in S_t)\mid \cG]\\
    & \leq \frac{1}{m}\sum_{i=1}^K \E\biggsn{\sum_{n=1}^{n_i(T)} (\theta_{i,t}^{\ucb} - \theta_i)\1(i \in S_t) \mid \cG }\\
    & \leq \frac{1}{m}\sum_{i=1}^K \E\biggsn{\sum_{n=1}^{n_i(T)} (\theta_{i,t}^{\ucb} - \theta_i)\1(i \in S_t) \mid \cG }\\
    & \leq \frac{1}{m}\sum_{i=1}^K \E\biggsn{\sum_{n=1}^{n_{i0}^{\text{init}}} (\theta_{i,t}^{\ucb} - \theta_i)\1(i \in S_t) + \sum_{n=n_{i0}^{\text{init}}+1}^{n_i(T)} (\theta_{i,t}^{\ucb} - \theta_i)\1(i \in S_t) \mid \cG }\\
    & \leq \frac{1}{m}\sum_{i=1}^K \E\biggsn{\sum_{n=1}^{n_i(T)} \frac{\sqrt{\log KT}}{\sqrt{n_{i0}(n)}} \mid \cG }\\
    &\overset{(a)}{\lesssim} \frac{1}{m}\sum_{i=1}^K \E\biggsn{\sum_{n =1}^{ n_{i}(T) } \frac{\sqrt{\log KT}}{\sqrt{n/m}} }\\
    &\overset{(b)}\leq \frac{1}{m}\E\biggsn{\sum_{i=1}^K {\sqrt{m n_i(T) }\log KT} }\\
    & \overset{(c)}\leq \frac{1}{m}\E\biggsn{{m\sqrt{K T} \log KT} } = \sqrt{KT}\log (KT),
\end{align*}

where (a) follows by noting that $\E[n_{i0,T}] \geq \frac{1}{m}\E[n_i(T)]$ w.h.p. $(1-1/{KT})$ at each round $t$ -- this is since the number of times either $i$ or $0$ won has to be at least $m$-factor of the total number of times item-$i$ was pulled. (b) and (c) simply follows by applying Cauchy's Schwarz Inequality with the additional observation that $\E[\sum_{i = 1}^K n_i(T)] \leq mT$.

\red{make a note on complications: getting rid of the m dependencies }

\end{proof}

\subsection{Analysis: \utilm\ Objective with \wf\ Feedback}
\label{sec:alg_wiutil_analys}

Let us denote by

\[
\cW_S:= \frac{\sum_{i \in S}w_i \theta_i}{\Theta_{S}+1}, ~\text{ and }  \cW^{\ucb}_{S,t}:= \frac{\sum_{i \in S}w_i \theta_{i,t}^{\ucb}}{\Theta_{S,t}^{\ucb}+1}.
\]

The first claim is to show that $\cW^{\ucb}_{S,t} \geq \cW_S, \forall S \subseteq [K]$. More formally,  

\begin{lemma}[Wtd-Utility UCB]
\label{lem:wtd_util}
Let $w_1,\dots,w_K >0$ and $t\in [T]$. Then, if Inequality~\eqref{eq:ucb_p1} holds for all couples $(i,0)$, it yields $\cW_{S,t}^{\ucb} \geq \cW_S$ for all $S$.
\end{lemma}

%{Proof is straightforward with induction, we moved it to the appendix for completeness}

\begin{proof}[Proof of \cref{lem:wtd_util}]
    The proof is straightforward. \red{complete}
\end{proof}

\begin{restatable}[\algwf: Regret Analysis for \utilm\ with \wf\ Feedback]{theorem}{utilmwf}
\label{thm:utilm_wf}
Consider any instance of PL model on $K$ items with parameters $(\theta_1,\ldots,\theta_K)$ and let $w_i > 0$ be the weight associated to item-$i$, forall $i \in [K]$. Then given any finite time horizon $T$, the weighted regret of our proposed algorithm \algwf\ is bounded as $\regu_T = O(\sqrt{KT\log KT})$. 
\end{restatable}

\begin{rem}
Say how we do against MNL Bandits \cite{assort-mnl} + Brag we improve since we use a better and simpler estimation and concentration bound, which they could not figure out and kept playing the same set again and again until the `no-choice' (item-$0$) gets selected.
\end{rem}

\begin{proof}[(Proof Sketch of \cref{thm:utilm_wf})]
We need to be a little more careful about the denominator for this case (since $1/m$ in the regret objective saved us from dealing with the extra $m$-factor in the \topm\ objective)

Now since, $\cW_{S^*} \leq \cW_{S^*,t}^{\ucb} \leq \cW_{S_t,t}^{\ucb}$, note we can write:

\begin{align*}
   \regu_T & = \sum_{t=1}^T \E\bigsn{\cW_{S^*} - \cW_{S_t}}  
    \leq \sum_{t = 1}^T \E\bigsn{\cW_{S_t,t}^{\ucb} - \cW_{S_t}}\\
    & \leq \sum_{t=1}^T  \E\biggsn{\sum_{i\in S_t} \frac{\theta_{i,t}^{\ucb} - \theta_i}{\Theta_{S_t}+1}}\\
    & \leq \sum_{t=1}^T \sum_{i\in S_t} \E\biggsn{\frac{(1+\theta_i)\sqrt{\theta_i x}}{\sqrt{(\Theta_{S_t}+1)^2 n_{i0,t}}}}\\
    & = \sum_{i=1}^K \sum_{t = 1}^T \E\biggsn{\frac{(1+\theta_i)\sqrt{\theta_i x}}{\sqrt{(\Theta_{S_t}+1)^2} \sqrt{n_{i0,t}}}}\1(i \in S_t)\\
    & = \sqrt{x} \sum_{i=1}^K \E\biggsn{ \sqrt{\sum_{t = 1}^T \frac{\theta_i }{(\Theta_{S_t}+1)}\1(i \in S_t)}} \times
    \sqrt{\E\biggsn{\sum_{t = 1}^T \frac{1 }{(\Theta_{S_t}+1) n_{i0,t}}  \1(i \in S_t)}} (1+\theta_i)\\
    & \text{since $\sqrt{\cdot}$ is convex, push $\E[\cdot]$ inside}\\
    & = \sqrt{x} \sum_{i=1}^K (1+\theta_i) \E\biggsn{ \sqrt{ \sum_{t = 1}^T \frac{\theta_i }{(\Theta_{S_t}+1)}\1(i \in S_t)}} \times
    \sqrt{\E\biggsn{\sum_{t = 1}^T\frac{1}{n_{i0,t}} \E[\1(i_t=0)\mid \1(i \in S_t)] \1(i \in S_t)}}\\
    %
    & = \sqrt{x} \sum_{i=1}^K(1+\theta_i) \E\biggsn{\sqrt{ \sum_{t = 1}^T \frac{\theta_i }{(\Theta_{S_t}+1)}\1(i \in S_t)}} \times
    \sqrt{\E\biggsn{ \sum_{t = 1}^{T}\frac{1}{n_{i0,t}} \E[\1(i_t=0)\mid \1(i \in S_t)] \1(i \in S_t)}}\\
    %
    & = \sqrt{x} \sum_{i=1}^K (1+\theta_i) \E\biggsn{\sqrt{ \sum_{t = 1}^T \frac{\theta_i }{(\Theta_{S_t}+1)}\1(i \in S_t)}} \times
    \sqrt{\E\biggsn{ \sum_{w = 1}^{w_0(T \mid i)}\frac{1}{w}}}\\
    &\leq  \sqrt{x \log T} \sum_{i=1}^K (1+\theta_i) \E\biggsn{\sqrt{ \sum_{t = 1}^T \frac{\theta_i }{(\Theta_{S_t}+1)}\1(i \in S_t)}}\\
    & \leq  \sqrt{x \log T} \sum_{i = 1}^K (1+\theta_i) \sqrt{\E\biggsn{ w_i(T)}} \\
    & \lesssim \theta_{\max} \sqrt{KT x}
    %
\end{align*}

\end{proof}

\begin{proof}[\red{(New proof)}]
    $W_{S,t}^{\text{ucb}} \geq W_{S,t}$, where the upper-bound on $\gamma_{ij,t}^{\text{ucb}}$ will be valid for $n_{ij,t} \geq C x (1 + \gamma_{ij})$. Let $j_t = \argmax_{j \in S_t} \theta_j$.

\begin{align*}
   & \regu_T  = \sum_{t=1}^T \E\bigsn{\cW_{S^*} - \cW_{S_t}}  
    \leq \sum_{t = 1}^T \E\bigsn{\cW_{S_t,t}^{\ucb} - \cW_{S_t}}\\
    & \leq \sum_{t=1}^T  \E\biggsn{ \min_j \sum_{i\in S_t} \frac{\gamma_{ij,t}^{\ucb} }{\gamma_{0j,t}^\ucb + \sum_{i \in S_t} \gamma_{ij,t}^\ucb} - \frac{\gamma_{ij} }{\gamma_{0j} + \sum_{i \in S_t} \gamma_{ij}} }\\
    & \leq \sum_{t=1}^T  \E\biggsn{  \sum_{i\in S_t} \frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} }\\
    & \leq   \sum_{i=1}^K \E\biggsn{   \sum_{t=1}^T  \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)\indic\{i \in S_t\}} \\
    & \leq  \sum_{i=1}^K \sqrt{ \sum_{t=1}^T \E \Bigg[ \frac{\gamma_{ij_t} \indic\{i \in S_t\}}{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \Bigg] }\\
    & \qquad \times \sqrt{\sum_{t=1}^T \E \Bigg[ \frac{1}{\gamma_{ij_t}}\bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i \in S_t\} 
 \Bigg]} \\
    & \leq   \sum_{i=1}^K \sqrt{ \E \big[w_{i,T}\big]} \\
    & \qquad \times \sqrt{\sum_{t=1}^T \E \Bigg[\frac{1}{\gamma_{ij_t}} \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i\in S_t\} 
 \Bigg]}
\end{align*}
But
\begin{align*}
\sum_{t=1}^T \E \Bigg[& \frac{1}{\gamma_{ij_t}} \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i \in S_t\} 
 \Bigg] \\
 & \leq \sum_{t=1}^T \E \Bigg[\frac{1}{\gamma_{ij_t}}  \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i,j_t \in S_t\} | \cE
 \Bigg]  + T M \delta  \\
 & \leq \sum_{t=1}^T \E \Bigg[\frac{1}{\gamma_{ij_t}}  \frac{(\gamma_{ij_t,t}^\ucb - \gamma_{ij_t})^2 }{\gamma_{0j_t} + \sum_{i,j_t \in S_t} \gamma_{ij_t}}  \indic\{i \in S_t\} | \cE
 \Bigg] \P(\cE) + T M \delta  \\
 & \leq \sum_{t=1}^T \E \Bigg[ \frac{ (1+\gamma_{ij_t})^2 x  \indic\{i \in S_t\}}{n_{ij_t,t}(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t} )} \Bigg| \cE \Bigg]\P(\cE) + T M \delta   \\
 & \leq \sum_{t=1}^T \E \Bigg[ \frac{ (1+\gamma_{ij_t}) x  \indic\{i\in S_t\}}{n_{ij_t,t}(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t} )} \Bigg] + T M \delta  \\
 & \leq 2x  \E \Bigg[ \sum_{t=1}^T \frac{  \indic\{i_t^* \in \{i,j_t\}, i\in S_t\}}{n_{ij_t,t}} \Bigg] + T M \delta \\
 & \leq 2x \sum_{t=1}^T \E \Bigg[ \sum_{j=0}^K \sum_{t=1}^T \frac{  \indic\{i_t^* \in \{i,j\}, i\in S_t\}}{n_{ij,t}}  \indic\{j = j_t\} \Bigg] + T M \delta  \,.
\end{align*}
\end{proof}

\newpage

\section{Algorithm for adapting to $\theta_{\max}$}

Denote $\gamma_{ij} = \frac{\theta_i}{\theta_j}$ and
$\gamma_{ij,t}^{\text{ucb}} = \frac{p_{ij,t}^{\text{ucb}}}{(1-p_{ij,t}^{\text{ucb}})_+}$. For all $S \subset [K]$ denote
\[
 W_{S,t}^\text{ucb} := \min_{j \in \{0\}\cup [K]} \frac{\sum_{i \in S} \gamma_{ij,t}^{\text{ucb}}}{\gamma_{0j,t}^{\text{ucb}} + \sum_{i \in S} \gamma_{ij,t}^{\text{ucb}}} \,.
\]
At round $t$, let the algorithm plays
\[
    S_t = \argmax_{S}  W_{S,t}^{\text{ucb}}\,.
\]
Note that this might be hard to solve...
Similarly to before, for all $(i,j)$ with high probability
\[
    \gamma_{ij} \leq \gamma_{ij,t}^{\text{ucb}} \leq \gamma_{ij} + 4(\gamma_{ij} + 1) \sqrt{\frac{2 \gamma_{ij} x}{n_{ij,t}}} + \frac{22 x (\gamma_{ij} + 1)^2}{n_{ij,t}} \,.
\]
and $W_{S,t}^{\text{ucb}} \geq W_{S,t}$, where the upper-bound on $\gamma_{ij,t}^{\text{ucb}}$ will be valid for $n_{ij,t} \geq C x (1 + \gamma_{ij})$. Let $j_t = \argmax_{j \in S_t} \theta_j$.

\begin{align*}
   & \regu_T  = \sum_{t=1}^T \E\bigsn{\cW_{S^*} - \cW_{S_t}}  
    \leq \sum_{t = 1}^T \E\bigsn{\cW_{S_t,t}^{\ucb} - \cW_{S_t}}\\
    & \leq \sum_{t=1}^T  \E\biggsn{ \min_j \sum_{i\in S_t} \frac{\gamma_{ij,t}^{\ucb} }{\gamma_{0j,t}^\ucb + \sum_{i \in S_t} \gamma_{ij,t}^\ucb} - \frac{\gamma_{ij} }{\gamma_{0j} + \sum_{i \in S_t} \gamma_{ij}} }\\
    & \leq \sum_{t=1}^T  \E\biggsn{  \sum_{i\in S_t} \frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} }\\
    & \leq   \sum_{i=1}^K \E\biggsn{   \sum_{t=1}^T  \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)\indic\{i \in S_t\}} \\
    & \leq  \sum_{i=1}^K \sqrt{ \sum_{t=1}^T \E \Bigg[ \frac{\gamma_{ij_t} \indic\{i \in S_t\}}{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \Bigg] }\\
    & \qquad \times \sqrt{\sum_{t=1}^T \E \Bigg[ \frac{1}{\gamma_{ij_t}}\bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i \in S_t\} 
 \Bigg]} \\
    & \leq   \sum_{i=1}^K \sqrt{ \E \big[w_{i,T}\big]} \\
    & \qquad \times \sqrt{\sum_{t=1}^T \E \Bigg[\frac{1}{\gamma_{ij_t}} \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i\in S_t\} 
 \Bigg]}
\end{align*}
But
\begin{align*}
\sum_{t=1}^T \E \Bigg[& \frac{1}{\gamma_{ij_t}} \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i \in S_t\} 
 \Bigg] \\
 & \leq \sum_{t=1}^T \E \Bigg[\frac{1}{\gamma_{ij_t}}  \bigg(\frac{\gamma_{ij_t,t}^{\ucb} }{\gamma_{0j_t,t}^\ucb + \sum_{i \in S_t} \gamma_{ij_t,t}^\ucb} - \frac{\gamma_{ij_t} }{\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}} \bigg)^2 \Big(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t}\Big) \indic\{i,j_t \in S_t\} | \cE
 \Bigg]  + T M \delta  \\
 & \leq \sum_{t=1}^T \E \Bigg[\frac{1}{\gamma_{ij_t}}  \frac{(\gamma_{ij_t,t}^\ucb - \gamma_{ij_t})^2 }{\gamma_{0j_t} + \sum_{i,j_t \in S_t} \gamma_{ij_t}}  \indic\{i \in S_t\} | \cE
 \Bigg] \P(\cE) + T M \delta  \\
 & \leq \sum_{t=1}^T \E \Bigg[ \frac{ (1+\gamma_{ij_t})^2 x  \indic\{i \in S_t\}}{n_{ij_t,t}(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t} )} \Bigg| \cE \Bigg]\P(\cE) + T M \delta   \\
 & \leq \sum_{t=1}^T \E \Bigg[ \frac{ (1+\gamma_{ij_t}) x  \indic\{i\in S_t\}}{n_{ij_t,t}(\gamma_{0j_t} + \sum_{i \in S_t} \gamma_{ij_t} )} \Bigg] + T M \delta  \\
 & \leq 2x  \E \Bigg[ \sum_{t=1}^T \frac{  \indic\{i_t^* \in \{i,j_t\}, i\in S_t\}}{n_{ij_t,t}} \Bigg] + T M \delta \\
 & \leq 2x \sum_{t=1}^T \E \Bigg[ \sum_{j=0}^K \sum_{t=1}^T \frac{  \indic\{i_t^* \in \{i,j\}, i\in S_t\}}{n_{ij,t}}  \indic\{j = j_t\} \Bigg] + T M \delta  \,.
\end{align*}

\iffalse%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
It is precisely the \emph{pivoting-trick} that helps up to circumvent an $O(n^k)$ combinatorial explosion that would otherwise result if we directly attempted to estimate probability distributions for each possible $k$-size subsets. The sample complexity of our resulting algorithms are $O\Big(   \frac{n}{\epsilon^2} \ln \frac{n}{\delta}\Big)$ which are in fact orderwise optimal as reflects from our derived lower bound guarantees in the next section (see Theorem \ref{thm:lb_plpac_win}). Moreover, in the dueling bandit setup for $k = 2$, our algorithms give an improvement by an additive factor of $\frac{n\log n}{\epsilon^2}\ln \frac{1}{\epsilon}$ compared to the state of the art algorithm by \cite{Busa_pl} that requires a sample complexity of $O\Big( \frac{n \ln n}{\epsilon^2} \ln \frac{n}{\epsilon\delta}\Big)$ --- the improvement precisely stems from the fact that unlike the previous approach, we here alleviate the overhead of maintaining $O(n^2)$ pairwise score estimates by the \emph{pivoting-trick} along with the novel parameter estimation results derived in Section \ref{sec:est_pl_score}. The formal description of our algorithms are given below:

\vspace*{5pt}
\noindent {\bf Principles of algorithm design.} The key idea on which all our learning algorithms are based is that of maintaining estimates of the pairwise win-loss probabilities $p_{ij} = Pr(i|{i,j})$ in the Plackett-Luce model. This helps circumvent an $O(n^k)$ combinatorial explosion that would otherwise result if we directly attempted to estimate probability distributions for each possible $k$-size subset. However, it is not obvious if consistent and tight pairwise estimates can be constructed in a general subset-wise choice model, but the special form of the Plackett-Luce model again comes to our rescue. The IIA property that the PL model enjoys allows for accurate pairwise estimates via interpretation of partial preference feedback as a set of pairwise preferences, e.g., a winner $a$ sampled from among ${a,b,c}$ is interpreted as the pairwise preferences $a \succ b$, $a \succ c$. Lemma \ref{lem:pl_simulator} formalizes this property and allows us to use pairwise win/loss probability estimators with explicit confidence intervals for them.

\begin{rem}
{
The sample complexity bound of Theorem \ref{thm:batt_giant} holds good for any IIA based choice model (PL model in particular), since its proof is based on Lemma \ref{lem:pl_simulator} and the observation made in Remark \ref{rem:iia_gen}.}
\end{rem}
\fi %%%%%%%%%%%%%%%%%%%%%%%%



==> relworks.tex <==
\subsection{Related Works}
\label{sec:relworks}

%\red{needs some more emphasize on assortment literature}

%For classical multiarmed bandits setting, there is a well studied literature on PAC-arm identification problem \citep{Even+06,Audibert+10,Kalyanakrishnan+12,Karnin+13,LilUCB}, where the learner gets to see a noisy draw of absolute reward feedback of an arm upon playing a single arm per round. 

Learning to identify the best item(s) with relative preference information (ordinal as opposed to cardinal feedback) has seen steady progress since the introduction of the dueling bandit framework \citep{Yue+12,Zoghi+14RCS} with pairs of items (size-$2$ subsets). Subsequent works generalized the setup to broader models both in terms of distributional parameters \citep{Yue+09,Adv_DB,Ailon+14, Zoghi+15MRUCB,ADB} as well as combinatorial subset-wise plays \citep{MohajerIcml+17,pbo,SG18,Sui+17,Busa21survey}. 
There have been several developments on the PAC objective for different pairwise preference models, such as those satisfying stochastic triangle inequalities and strong stochastic transitivity \citep{BTM}, general utility-based preference models \citep{SAVAGE}, the Plackett-Luce model \citep{Busa_pl} and the Mallows model \citep{Busa_mallows}]. %Recent work has studied PAC-learning objectives other than identifying the single (near) best arm, e.g. recovering a few of the top arms \citep{Busa_top,MohajerIcml+17}, or the true ranking of the items \citep{Busa_aaai,falahatgar_nips}. 

Some of the recent works also extended the pairwise (dueling) feedback objective to relative subsetwise preferences \citep{SGrank18,ChenSoda+17,ChenSoda+18,SGwin18,Ren+18,SGinst20,SGrum20}.
However, the majority of these works have primarily focused on the objective of either identifying optimal items within a PAC (probably approximately correct) framework or quantifying regret concerning a predetermined best item. These approaches, while theoretically insightful, involve practical challenges from a real-world perspective. Clearly, recovering a set of the top-rank items or the full ranking makes more sense for any practical system, which however has not been considered in any of the prior works with an active regret minimization objective. 

%However, none of the existing work considers strategies to learn efficiently in general RUMs with subset-wise preferences and to the best of our knowledge we are the first to address this general problem setup. 
In a different direction, there has been some work on batch (non-adaptive) estimation in general RUMs, e.g., \citep{zhao2018learning,soufiani2013generalized}; however, this does not consider the price of active learning and the associated exploration effort required as we study here. Another related body of literature lies in dynamic assortment selection, where the goal is to offer a subset of items to customers in order to maximize expected revenue, which has been studied under different choice models, e.g. Multinomial-Logit \citep{assort-mnl}, Mallows and mixture of Mallows \citep{assort-mallows}, Markov chain-based choice models \citep{assort-markov}, single transition model \citep{assort-stm} etc. While these works indeed consider a more practical objective of finding the best assortment (subset) with the highest utility for a regret minimization objective, a major drawback in their approach lies in the algorithm design which requires to keep on querying the same set multiple times, e.g. \cite{assort-mnl,ou2018multinomial,assort-nested}. Such design techniques could be impractical to be deployed in real systems where users could easily get annoyed if the same items are shown again and again.  As discussed in our list of contributions above, our proposed algorithms overcome this problem with a novel parameter estimation technique for discrete choice models and yield a computationally efficient and regret optimal algorithm for different types of preference feedback.

==> res.tex <==
\section{Experiments}

\section{Conclusion and future work}

\iffalse%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Questions/Ideas}

\begin{itemize}[nosep]
    \item Battling bandit with more arms
    \item Improving the dependence on $K$
    \item Applying the result of Zimmert with OMD to achieve gap dependent bounds.
    \item Showing that sleeping internal regret implies ordering regret for i.i.d. availabilities.
    \item 
\end{itemize}


Now Pierre writing: Can we come up with an algorithm for low internal regret with sleeping bandits for MAB. Once we have the result for MAB, we can do the reduction idea to get the "low" internal regret algorithm for DB. 

We already show (Lem): 1. For stochastic losses and stoc sleeping,  "low" internal regret implies "low" ordering regret (as well as low policy regret)
 
 

Yet to solve:---

1. For stochastic sleeping and adversarial losses, does "low" internal regret implies "low" ordering regret ?

2. For stochastic sleeping and adversarial losses, (where losses/ rewards are chosen independent of the subset availabilities), does ordering regret (this paper) and policy regret (ICML20 paper) equivalent of the later is stronger?

3. 

Expts:

MAB: 3 algos) Klienberg (stoc rewards \& adv sleeping), ICML20 (other way), and our internal regret based algorithm

>> Settings: (a) Stoc rew and adv sleeping (b)  Adv rew and stoc sleeping

DB1: Compare Neurips paper vs our reduction+internal regret (for Stoc rew and adv sleeping)

DB2: Reduction+ICML20 --- Compare performance of DB1 with 

\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
